Flatter is better: Percentile Transformations for Recommender Systems

It is well known that explicit user ratings in recommender systems are biased towards high ratings, and that users differ significantly in their usage of the rating scale. Implementers usually compensate for these issues through rating normalization or the inclusion of a user bias term in factorization models. However, these methods adjust only for the central tendency of users' distributions. In this work, we demonstrate that lack of \textit{flatness} in rating distributions is negatively correlated with recommendation performance. We propose a rating transformation model that compensates for skew in the rating distribution as well as its central tendency by converting ratings into percentile values as a pre-processing step before recommendation generation. This transformation flattens the rating distribution, better compensates for differences in rating distributions, and improves recommendation performance. We also show a smoothed version of this transformation designed to yield more intuitive results for users with very narrow rating distributions. A comprehensive set of experiments show improved ranking performance for these percentile transformations with state-of-the-art recommendation algorithms in four real-world data sets.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> body-v01.tex <==
\section{Introduction}


Recommender systems have become an essential tool in e-commerce systems, helping users to find desired items in many contexts. These systems use information from user profiles to generate personalized recommendations. User profiles are either implicitly inferred by the system through user interaction, or explicitly provided by users \cite{Adomavicius:2005,Adomavicius:2015}. In the latter case, users are asked to rate different items based on their preferences and may have individual differences in how they use explicit rating scales: some users may tend to rate higher, while some users may tend to rate lower; some users may use the full extent of the rating scale, while others might use just a small subset. \cite{Herlocker:1999a}. 

When a user concentrates his or her ratings in only small subset of the rating scale, we often end up with ratings distributions that are skewed -- most often towards the high end of the scale. This is because items are not rated at random, but rather preferred items are more likely to be experienced and therefore rated due to selection bias~\cite{marlin2007collaborative}. Figure \ref{fig1} shows the overall rating distribution of two data sets that exhibit typically right-skewed distributions. Users in CiaoDVD data set, for example, have assigned less than 10\% of the ratings to ratings 1 and 2 and some 70\% of ratings are values 4 and 5. We can assume this is not because there are so many more good movies than bad, but rather than users are selecting movies to view that they are likely to enjoy and the ratings are concentrated among those selections. A drawback of this skew to the distribution is that we have more information about preferred items and less information about items that are not liked as well. 

\addtolength{\parskip}{-0.5mm}
\begin{table}[t]
\centering
\captionof{table}{\label{tab:example} Rating profiles with percentile transformation}
\begin{tabular}{ l | l | l}
\hline
Alice & rating & $\langle 1,1,2,2,3,3,3,4,5 \rangle$ \\
Bob & rating & $\langle 3,3,4,4,4,5,5,5,5 \rangle$ \\
\hline
Alice & percentile & $\langle 20,20,40,40,70,70,70,80,90 \rangle$ \\
Bob & percentile & $\langle 20,20,50,50,50,90,90,90,90 \rangle$\\
\hline
\end{tabular}
\end{table}


\begin{figure} 
\includegraphics[height=2in, width=3in]{distribution.png}
\caption{Rating distribution of CiaoDVD and MovieLens data sets.}\label{fig1}
\end{figure}

Moreover, similar issue can be observed on items which is well-known as \textit{item popularity}. Item popularity refers to the fact that depending on what recommendation algorithm we apply, inherent popularity bias in input data causes algorithms to focus their recommendations on a small set of items. Because often the items of greatest interest to users are the lesser-known ones~\cite{longtailnichesriche, park}, but these items are less common in recommendation lists -- a consequence of lack coverage of the items across the catalog. Low catalog coverage has several consequences: (1) the system may miss good items which otherwise would improve the accuracy and users' satisfaction, and items belonging to some providers may never have chance to be recommended, which is not fair for those providers. An ideal recommendation system would be one that, while accurate, allows all items regardless of their popularity to have an equal chance of appearing in recommendation lists. 

%\begin{figure*}[!tbp]
%  \begin{subfigure}[b]{0.25\textwidth}
%    \includegraphics[width=\textwidth]{rate-biasedmf-log.png}
%    \caption{Biased MF}
%    \label{fig:f1}
%  \end{subfigure}
%  \hfill
  %\begin{subfigure}[b]{0.24\textwidth}
  %  \includegraphics[width=\textwidth]{rate-listrank.png}
  %  \caption{ListRank MF}
  %  \label{fig:f2}
  %\end{subfigure}
  %\hfill
%  \begin{subfigure}[b]{0.25\textwidth}
%    \includegraphics[width=\textwidth]{rate-svdpp-log.png}
%    \caption{SVD++}
%    \label{fig:f2}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[b]{0.29\textwidth}
%    \includegraphics[width=\textwidth]{rate-itemknn-log.png}
%    \caption{ItemKNN}
%    \label{fig:f2}
%  \end{subfigure}
%  \hfill
  %\begin{subfigure}[b]{0.33\textwidth}
  %  \includegraphics[width=\textwidth]{rate-userknn-log.png}
  %  \caption{UserKNN}
  %  \label{fig:f2}
  %\end{subfigure}
%  \caption{Popularity of items versus frequency of recommendation for different recommendation algorithms on Yelp data set, list length 10. Log-log scale.} \label{fig2}
%\end{figure*}

%Figure \ref{fig2} compares the behavior of several recommendation algorithms on recommending businesses in our Yelp data set across the popularity distribution. In these scatter plots with log-log scaling, points represent items in the catalog, distributed on the horizontal axis from least to most popular. The vertical axis is the percentage of times each item appeared in recommendation lists across all users. As shown in this figure, recommendation algorithms cover various fractions of items. Factorization models (such as Biased Matrix Factorization and SVD++ reported here) are more likely to recommend items at the lower end of the distribution, while neighborhood models mainly tend to have greater concentration on popular items. (We observed similar result on \algname{UserKNN}.) Note also that factorization models recommend fewer items but recommend them more frequently -- note the cloud of frequently recommended items -- while the neighborhood model does not have such items. These results are consistent with the findings in \cite{Jannach2015, coba2017} 

A drawback of skew to the rating distribution is that we have more information about preferred items and less information about items that are not liked as well. One can imagine an ideal rating distribution would a flat, uniform, distribution. Users would sample uniformly across all of the items and the profiles would then represent preferences across the whole inventory, and across all possible rating values. %One can imagine the most informative rating distribution would be a flat, uniform, distribution. Users would sample uniformly across all of the items and the profiles would then represent preferences across the whole inventory, and across all possible rating values. One way to think about the difference between the typical, skewed, distribution and a uniform one is in terms of information entropy. The worst case, a profile where every item is rated the same, carries no information that distinguishes the different items, and the assignment of a rating to an item has low entropy. A profile where the rating values are distributed across the items with equal frequency has maximum entropy.

In this paper, we propose a rating transformation model that converts users' ratings into percentile values as a pre-processing step before recommendation generation. Each value associated with an item therefore reflects its rank among all of the items that the user has rated. Thus, the percentile captures an item's position within a user's profile better than the raw rating value and therefore compensates for differences in users' overall rating behavior. Also, the percentile, by definition, will span the whole range of rating values, and as we show, gives rise to a more uniform rating distribution.

We show that these two properties of the percentile transformation -- its ability to compensate for individual user biases and its ability to create a more uniform rating distribution -- lead to enhanced recommender system performance across a range of different algorithms, different data sets, and different performance measures. We also show that the percentile transformation creates flatter rating distributions and that this is correlated with improved recommendation performance.

We demonstrate the effectiveness of the proposed percentile technique using multiple recommendation algorithms on six publicly-available data sets in terms of ranking quality and item coverage.

Overall, our paper makes the following contributions:

\begin{enumerate}[\hspace{0.4cm}1.]
  \item We propose a rating transformation model that converts users' ratings into percentile values to compensate for skew in rating distributions and variances in users' rating behaviors.
  \item We empirically evaluate the proposed percentile technique using state-of-the-art recommendation algorithms on four real-world data sets.
  \item We show the relationship between the uniformity of the rating distribution and the quality of recommendation; with flatter distributions being correlated with better recommendations.
\end{enumerate}




% Head 2
\section{Background}

\subsection{User bias}
\noindent It has long been noted that users differ in their application of explicit rating scales. Resnick's algorithm, perhaps the most well-known prediction method in recommendation, normalizes ratings by user mean when computing its predictions~\cite{Resnick:1994a}. Herlocker, et al. \cite{Herlocker:1999a} used z-scores instead of absolute rating values in recommender systems and investigated its effectiveness on quality of recommendations. In this research they compared the performance of three rating normalization techniques and showed that bias-from-mean approach performs significantly better than a non-normalized rating approach and slightly better than the z-score approach in terms of mean absolute error. This is a consistent result with the results in this paper. 

Kamishima in \cite{Kamishima:2010} proposed a ranking-based method that replaces the existing rating scheme with a ranking scheme. In this method, instead of rating the items, users order the items based on their preferences. Based on order statistics theory, preference orders expressed by users are converted into scores and then recommendation algorithms are applied on these scores to generate recommendations. This method proved effective, but it is not widely applicable because order-based input is rare in recommender system interfaces, and requires more effort from users than rating assignment. 

Jin, et al. \cite{Jin:2004a} compared the impact of two normalization techniques for user ratings, namely Gaussian and decoupling normalization techniques on the performance of recommender systems. This research found that decoupling normalization is more effective than Gaussian normalization. A more recent study by \cite{Kim:2016a} proposed a normalization model that learns the differences in users' rating dispositions using two phases of clustering and normalization. At the clustering phase, users are clustered based on their rating disposition and then at the normalization phase, users' ratings are normalized through predicting their rating disposition and adjusting their neighbors' ratings based on that disposition.

\subsection{Item popularity}

Jannach et. al., \cite{Jannach2015} conducted a comprehensive set of analysis on popularity bias of several recommendation algorithms. They analyzed recommended items by different recommendation algorithms in terms of their average ratings and their popularity. While it is very dependent to the characteristics of the data sets, they found that some algorithms (e.g., \algname{SlopeOne}, KNN techniques, and ALS-variant of factorization models) focus mostly on high-rated items which bias them toward a small sets of items (low coverage). Also, they found that some algorithms (e.g., ALS-variants of factorization model) tend to recommend popular items, while some other algorithms (e.g., \algname{UserKNN} and \algname{SlopeOne}) tend to recommend less-popular items. These results are very consistent with our results and findings in this paper. One of our claim in this paper is that presence of high-rated items negatively affect recommendation performance on covering items in recommendation lists. We show that the proposed transformation model properly compensate for high-rated items. Also, results presented in \cite{coba2017} showed that \algname{UserKNN} tend to recommend short-head items, while \algname{ItemKNN} tend to recommend long-tail items Which, again, are consistent with our observation in Figure \ref{fig2}.

Abdollahpouri et. al., \cite{himan2017} addressed popularity bias in learning-to-rank algorithms by inclusion of fairness-aware regularization term into objective function. They showed that the fairness-aware regularization term controls the recommendations being toward popular items. Also, Steck in \cite{harald2011} examined the trade-off between degrading accuracy for improving long-tail coverage. By conducting user study, they observed that adding a small bias toward long-tail items leads to better feedback from users.   

Ge et. al., \cite{ge2010} analyzed the trade-off between coverage and serendipity of the recommendations and proposed a new way of measuring these metrics. In their proposed measurements, the usefulness of an item is incorporated to measure the coverage and serendipity in a way to enhance the quality of recommendations.




% Head 3
\section{Percentile transformation}

In statistics, given a series of measurements, percentile (or quantile) methods are used to estimate the value corresponding to a certain percentile. Given the \textit{P}\textsuperscript{th} percentile, these methods attempt to put \textit{P}\% of the data set below and (100-\textit{P})\% of the data set above. There are a number of different definitions in the literature for computing percentiles \cite{Hyndman:1996,Langford:2006}. Although they are apparently different, the answers produced by these methods are very similar and the slight differences are negligible \cite{Langford:2006}. In this paper, we use a definition from \cite{Hyndman:1996} .

The percentile value, \(p\), corresponding to a measurement, \(x\), in a series of measurements, \(M\), is computed with regard to the position of \(x\) in the ordered list \(M\), \(o(M)\), as follows: 

\begin{equation} \label{eq:percentile}
p^z(x,M)=\frac{100\times position^z(x,o(M))}{|M|+1}
\end{equation}
where \(position^z(x, o(M))\) returns the index of occurrence of \(x\) in \(o(M)\), or the position in the order where $x$ would appear if it is not present, and \(|M|\) is the number of measurements in \(M\). For more details see \cite{Hyndman:1996}.

This transformation assumes that values are distinct and there is no repetition in the series. However, with explicit rating data, we have a different situation. User profiles usually contain many repetitive ratings, and it is unclear how to specify the position of a rating. For example, in a series of ratings $v=\langle 2, 3, 3, 3, 3, 3, 5, 5, 5 \rangle$, it is not clear what the position of rating 3 should be. We could take the first occurrence, position 2, or the last occurrence 6, or something in between. 

In this work, we explore the performance of our percentile technique by taking the index of the first, median, and last occurrence of repeated ratings in the ordered vector. Hence, the parameter $z$ determines the index rule that we want to use for percentile transformation and can take values $f$, $m$, and $l$ as $first$, $median$, and $last$ index assignments, respectively. Each of these index assignments signifies a particular meaning when transforming rating profiles. The index of the last occurrence, for example, is the highest rank (most preferred) position occupied by an item with the given rating. We experiment with all index assignments and show that the rule that yields a more uniform distribution will provide greater recommendation performance\footnote{See https://github.com/masoudmansoury/percentile for the code for computing the transformation.}. 

For our purposes, the entire set of ratings provided by a user \(u\) is considered a rating vector for \(u\), denoted by \(R_{u}\) with an individual rating for an item $i$, denoted as $r_{ui}$. Let $p(v,\ell)$ be the percentile mapping in Equation \ref{eq:percentile} from a rating value $v$ in a list of values $\ell$, using the first, median, and last index method. Then, the percentile value of a rating \(r\) provided by user \(u\) on an item \(i\) is computed by taking the rating $r_{ui}$ and calculating its percentile rank within the whole profile of the user. For example, based on the last index rule, for the user Bob from Table \ref{tab:example}, an item rated 3 would have percentile rank $100*2/(9+1) = 20$. We define the user-percentile function, $Per^z_u$, as follows:
\begin{equation} \label{eq:percu}
\mbox{Per}^z_u(u,i)= p^z(r_{ui}, R_u)
\end{equation}

Analogously, we can consider profiles for an item, denoted by $R_i$, to be all of the ratings provided for that item by users, and we can define a similar transformation for item profiles in which the transformation takes into consideration the rank of the rating across all ratings for that item, a item-percentile function:
\begin{equation} \label{eq:perci}
\mbox{Per}^z_i(u,i)= p^z(r_{ui}, R_i)
\end{equation}

Note that $Per^z_u$ and $Per^z_i$ might be quite different for the same user-item pair. For example, user $x$ might be a strong outlier relative to the data set, liking an item $y$ that no one else does. $Per^z_i(x,y)$ would therefore be quite high. However, if user $x$ has a strong tendency to high ratings in general, $Per^z_u(x,y)$ might be significantly lower. 

A drawback of the proposed percentile technique is conversion of identical ratings in a user's profile (e.g., <3,3,3,3,3,3>). When a user rates every item with the same rating values, it is hard to determine user's preferences and attitudes toward those items. Such rating profiles may be interpreted differently: if user A is a generous user (tends to rate highly) in rating items, rating 3 can be interpreted as \textit{like}, while if user A is a stingy user (tends to rate low) in rating items, rating 3 can be interpreted as \textit{dislike}. This issue is even more problematic in other transformation techniques like z-score as mean and standard deviation are not clear and accurate in this situation. To overcome this issue in our percentile technique, we introduce a \textit{smoothed percentile} technique.


\subsection{Smoothed percentile}

In smoothed percentile, we take into account the magnitude and frequency of identical ratings in the profile. This is done through adding a specific number of fake ratings to user's profile and then applying the proposed percentile technique on the updated rating profile. The number of fake ratings, $k$, that we add to a user's profile is a hyperparameter that needs to experimentally be determined. For adding fake ratings to a user's profile, first we take all rating members within the dataset and then we add a specific number of each rating member to user's profile. In 5-star rating system, for example, rating members are {1,2,3,4,5}. To transform <3,3,3> with $k=2$, adding fake ratings changes the rating profile to <1,1,2,2,3,3,3,3,3,4,4,5,5>. 

We formalize our smoothed percentile technique for each index assignment as follow:

\begin{equation} \label{eq:smoothedpercentilefirst}
p^f(x,M)=\frac{100\times (position^f(x,o(M)) + (k \times (index(x)-1)))}{|M|+(|R|*k)+1}
\end{equation}

\begin{equation} \label{eq:smoothedpercentileceil}
p^m(x,M)=\frac{100\times (position^m(x,o(M)) + (k \times (index(x)-1)) + k/2)}{|M|+(|R|*k)+1}
\end{equation}

\begin{equation} \label{eq:smoothedpercentilelast}
p^l(x,M)=\frac{100\times (position^l(x,o(M)) + (k \times index(x)))}{|M|+(|R|*k)+1}
\end{equation}

where $index(x)$ returns the index of rating $x$ in whole of ratings values within the data set. In rating system such as \{0.5,1,1.5,2,2.5,3\}, for example, $index(1)=2$ or $index(2.5)=5$. $|R|$ is the number of ratings member in the data set (i.e., in 5-star rating system, $|R|=5$).


\subsection{Measuring distribution uniformity} \label{flatness}

One of our claims is that the flatness of the rating distribution in a data set is an indicator of how well collaborative recommendation will perform, and that the percentile transformation achieves flatter distributions. In order to test this hypothesis, we need a measure of how close a rating distribution is to uniformity. 

To determine the flatness of a ratings distribution we calculate Kullback-Leibler divergence (KLD) between the observed rating distribution and a uniform distribution in which each rating value occurs the same number of times. If there is a discrete set of rating values $V$ (for example, {1,2,3,4,5}), then we define the flatness measure $\mathcal{F}$ as
\begin{equation}\label{eq:kldflat}
\mathcal{F}(D \parallel Q)=\sum_{v \in V} {D(v)\log\frac{D(v)}{Q(v)}}
\end{equation}
where $V$ is the set of discrete rating values in rating matrix $R$, and $D$ is the observed probability distribution over those values. $Q$ is a uniform distribution which associates a probability $1/|V|$ for each possible value in $V$ (i.e., for each $v \in V$, $Q(v)=1/|V|$). Therefore, 

\begin{equation}\label{eq:flat}
\mathcal{F}(D)=\sum_{v \in V} {D(v)\log(|V|D(v))}
\end{equation}

The $\mathcal{F}$ function measures the distance between the two distributions and hence how close the observed distribution is to the flat ideal, with a lower KLD value being indicative of a flatter distribution. 

Table \ref{tab:exflat} illustrates the flatness calculation of BookCrossing data set for original ratings. In this data set, there are ten rating values, $|V|=10$. $D(v)$ is the probability distribution over each rating values calculated as

\begin{equation}
D(v)=\frac{frequency(v)}{\sum_{v \in V}{frequency(v)}}
\end{equation}
By using equation \ref{eq:flat}, the flatness of this data set will be $\mathcal{F}=0.448$. Comparison between this flatness and the flatness of a uniform distribution (i.e., $\mathcal{F}=0$) shows that the distribution of original ratings in BookCrossing data set is far from a flat ideal. 

\input{1.KLDEX.tex}

The percentile and z-score transformations yield real valued ratings, unlike the original discrete ratings chosen by users in these data sets. Evaluating our flatness measure at every point in these distributions yields results that are not comparable to the original discrete distribution. 

In order to have comparable calculations of the $\mathcal{F}$ value across types of distributions, we created binned versions of the percentile and z-score distributions, using the same number of bins as present in the original ratings. In a 10-star rating system, such as found in the BookCrossing data, the rating distribution covers ten values, hence we created ten equal length bins for percentile and z-score values and aggregated each bin by its mean \footnote{As an example, we know that percentile values are between 0-100. Thus, we create ten bins each of which with the length of 10 and aggregate each bin by mean of its distribution.}. 

\begin{figure}[tbh] 
\includegraphics{bx-distribution-percentile.png}
\caption{Raw and binned percentile distributions for BookCrossing data set.\label{fig2}}
\end{figure}

Figure \ref{fig2} shows the percentile distribution (last index illustrated here) and its aggregated distribution for the BookCrossing data set. The black curve is the percentile distribution and red line is its aggregated distribution with ten bins. It shows that aggregating by mean retains the shape of the percentile distribution, while being comparable to the original ratings.


% Head 4
\section{Experiments}

\noindent We evaluated the performance of percentile transformation on four publicly available data sets: BookCrossing, CiaoDVD, FilmTrust, and MovieLens. The characteristics of the data sets are summarized in Table \ref{tab:dataset}. These data sets are from various domains and have different degrees of sparsity.

\input{2.dataset.tex}

The ML1M is movie ratings data and was collected by the MovieLens \footnote{https://grouplens.org/datasets/movielens/} research group. The CiaoDVD \footnote{https://www.cse.msu.edu/~tangjili/trust.html}  includes ratings of users for movies available on DVD. The FilmTrust is a small data set collected from FilmTrust website \cite{guo2013}. It contains both movie ratings and explicit trust ratings.
%The Epinions \footnote{http://www.trustlet.org/downloaded_epinions.html} data set was collected from Epinions web site which is an item reviewing system. It is a subset extracted from Epinions data set in which each user has rated at least 15 items and each item is rated by at least 15 users. The Yelp data set is a subset from the Yelp Challenge data set \footnote{https://www.yelp.com/dataset} in which users are rating businesses, often restaurants. In Yelp data set, each user has rated at least 5 reviews and each review is rated by at least 5 users. 
Finally, the BX data set is a subset extracted from the BookCrossing data set \footnote{http://www.informatik.uni-freiburg.de/\textasciitilde cziegler/BX/}  such that each user has rated at least 5 books and each book is rated by at least 5 users. The ML1M has the highest density and CiaoDVD has the lowest density.

\subsection{Flatness}

To evaluate the percentile transformation for its distributional properties, we evaluated its flatness compared to the original ratings 
distribution and a distribution based on the z-score transformation over four data sets: BX, CiaoDVD, FilmTrust, ML1M.

\input{3.kld.tex}

First, we converted the original ratings into percentile and z-score values. Then, we applied the binned flatness measure described above to these data sets to evaluate the transformations for their distributional properties. Table \ref{tab:kld} shows the $\mathcal{F}$ value for each type of transformation on the four data sets (note that transformations are based on users' profile). As anticipated, the proposed percentile model makes the rating values flatter than the original ratings and z-score values. Also, the original rating values show a flatter distribution than z-score values over all the data sets. 

Thus, the proposed percentile transformation approach reduces skew in the rating distribution over the original ratings and over z-score values. Given these results, we expect to see better recommendation performance when we use percentile values as input for recommender systems. We also expect that in most cases, using the original ratings will result in better recommendation performance than z-score values since they have lower $\mathcal{F}$ values.

\subsection{Methodology}

We performed a comprehensive evaluation of the effect of the percentile transformation on the ranking performance of multiple recommendation algorithms. Due to the nature of our percentile technique, experiments only on algorithms are reasonable that rating values (magnitude of ratings) are the core for those algorithms. Because our transformation technique only changes the rating values into a meaningful input for recommendation algorithms and does not have any impact on ranking order or binarized values of original ratings. Thus, recommendation algorithms that use ranking order or binarized value of ratings as input for recommender systems are not appropriate for our experiments. Also, for recommendation algorithms that rating values are implicitly or indirectly used for recommendation generation, our percentile technique will not significantly improve recommendation performance. In all those situations, rating transformation may not have much impact on recommendation outputs. This is also true about z-score transformation.

The algorithms that we experimented were non-personalized item average, user-based collaborative filtering \cite{Resnick:1994a}, item-based collaborative filtering \cite{sarwar2001}, biased matrix factorization \cite{Koren:2009a}, list-wise matrix factorization \cite{shi2010}, singular value decomposition \cite{Koren:2008a}, non-negative matrix factorization \cite{lee:2001}, and the sparse linear method \cite{Ning2011}. However, in this paper, for the purpose of expressive presentation, we only report results on biased matrix factorization (\algname{BiasedMF}) and singular value decomposition (\algname{SVD++}). On other recommendation algorithms, although results by our percentile transformation in most cases were better than original ratings and z-score transformation, those were not substantial. This is mainly due to the fact that in those algorithms the rating values are not the core for the algorithm and are not directly used in generating recommendation lists. In neighborhood model for ranking task \cite{mukund2004}, for example, rating values are used to calculate the similarity between users/items, and then only those similarity values are used for generating recommendation lists. 

We performed 5-fold cross validation for our experiments, and in the test condition, generated recommendation lists of size 10 for each user. Then, we evaluated nDCG and item coverage\footnote{We have also evaluated our results based on precision, recall, and F-measure. Analogous to nDCG and item coverage, we observed significant results on precision, recall, and F-measure.}, all at list size 10. Results were averaged over all users and then over all folds. A paired t-test was used to evaluate the significance of results and based on paired t-test, our results are statistically significant with a p-value of less than 0.05.

Before reporting on the results here, we performed extensive experiments with different parameter configurations for each algorithm and data set combinations. To determine sensible values for parameters, we followed the settings reported in the literature. In factorization models, for instance, we approximately set the number of factors and iterations based on the density of the data set and convergence of the loss function, and we tested these parameters for sensitivity. We performed a grid search over $bias\footnote{User, item, implicit feedback, and overall bias terms.} \in \{0.0001, 0.001, 0.005, 0.01\}$, $factor \in \{50, 100, 150\}$, $iteration \in \{30, 50, 100\}$, and $learning rate \in \{0.0001, 0.001, 0.005, 0.01\}$. 
%Sensitivity analysis is presented in the following section. 
Results of extensive experiments show that, in general, across on all settings, our percentile technique works significantly better than original ratings.  

%Note that this methodology is conservative, in that we are not optimizing the hyperparameters for the percentile distribution to get maximum performance. We are using the configuration that is optimal for the rating-based data. It is reasonable to expect, and some experimental evidence suggests, that even greater improvements could be achieved by these parameters, particularly the training iterations for the percentile data.
%In factorization models for the Yelp data set, for example, we conducted experiments with different number of factors from 50 to 300 and with different number of iterations from 20 to 100, choosing the settings for which each algorithm had the best performance. Although we report only on this best-performing configuration, we found that, in general, across on all settings, our percentile technique works significantly better than absolute rating values.

\subsection{Results}

\input{ndcg_table.tex}

There are ten experimental conditions: two recommendation algorithms evaluated over three different inputs: the original ratings, the results of the percentile transformation, and the results of z-score transformation; and two different transformation types: item-based and user-based transformations. Although in all situations our percentile technique works better than other input values, here we report user-based transformation to evaluate the recommendation performance in terms of ranking quality and item-based transformation to evaluate the recommendation performance in terms of item coverage. 
%For all recommendation algorithms except \algname{SLIM} and \algname{ItemAVG}, we used $Per_u$ to calculate the percentile values. \algname{SLIM} and \algname{ItemAVG} are item-based algorithms: therefore, percentile values are calculated based on $Per_i$. 
We used Lib\-Rec 2.0 to perform the experiments \cite{Guo2015}. 

Table \ref{tab:res1} shows the results for all the data sets and all algorithms. 
%Columns corresponding to \textit{params} present the parameters settings for recommendation algorithms. For \algname{UserKNN}, the parameter is the number of neighbors. For \algname{BiasedMF}, \algname{ListRank}, \algname{SVD++}, and \algname{NMF}, the parameters are the number of factors and the number of iterations, respectively. For \algname{SLIM}, the parameters are the $\ell_{1}$-norm and $\ell_{2}$-norm regularization weights. 
In this table, we report the best-performing configuration for each dataset, algorithm, and input value.
%, while results for different configurations are reported in sensitivity analysis section. 

Results shown in table \ref{tab:res1} show that percentile technique produces recommendations that are consistently better than original rating values over all the recommendation algorithms and data sets and all evaluation measures. %On \algname{BiasedMF}, \algname{ListRank}, and \algname{SVD++}, the percentile technique works significantly better with respect to all metrics showing improvement significant at the 99\% level. On \algname{NMF}, the percentile technique has better performance, which is significant at the 95\% level over all the data sets except BX.

%For \algname{UserKNN} algorithm, percentile transformation outperformed original ratings at 99\% level for denser data sets and 90\% level for sparser data sets. For this algorithm, density appears to have a significant impact on the results that can be obtained with the percentile transformation. We believe this is because larger profiles result in greater nuance being expressed through the percentile transformation, while shorter profiles are more likely to be similar to the original rating data. On ML1M, Yelp, and BX as the densest data sets, the percentile technique is significant mostly at 99\% level. On the sparser CiaoDVD data set, the percentile technique is significant at 90\% level.
%For the \algname{UserKNN} algorithm, density appears to have a significant impact on the results that can be obtained with the percentile transformation. We believe this is because larger profiles result in greater nuance being expressed through the percentile transformation, while shorter profiles are more likely to be similar to the original rating data. On ML1M as the densest data set, the percentile technique is significant at 95\% level. On the sparser Yelp data set, the percentile technique is significant almost at 90\% level. Less significant results are observed on BX and CiaoDVD, which are the sparsest data sets.

%\algname{SLIM} is an item-based algorithm, a generalization of item-based k-nearest neighbor. Since it is an item-based algorithm, we used $Per_i$ to calculate the percentile values. As shown in Table \ref{tab:res1}, on \algname{SLIM}, the percentile technique is significant at 90\% and 95\% level for some but not all measures, over the Yelp and CiaoDVD data sets, respectively, while it is not significantly better than non-transformed data over the other data sets, and for BX and MovieLens it is worse.
 
%Non-personalized item popularity (\algname{ItemAvg}) is another item-based recommendation algorithm, that recommends top-N items with the highest average rating. Like \algname{SLIM}, $Per_i$ is used to calculate the percentile values. Results show that our percentile technique on \algname{ItemAvg} works significantly better than the original rating values over all the data sets except BX.  

\subsection{Popularity analysis}

In this section, we examine the performance of recommendation algorithms in terms of catalog and long-tail coverage for different input values. Since there i always a trade-off between item coverage and ranking quality, we consider both when analyzing the effectiveness of recommender systems.
%Item popularity is well-known phenomena in recommender systems which refers to the fact that popular items are frequently recommended to users, while recommendation of less popular items is rare. This 

Given the whole set of items in the system as catalog, $C$, and whole recommendation lists for all users, $R_{all}$, catalog coverage (CC) measures what percentage of items in catalog appeared in recommendation lists and can be calculated as:

\begin{equation}
CC=100.\frac{|\{i, i \in (R_{all} \cap C)\}|}{|C|} 
\end{equation}

Also, the same equation can be used to calculated the long-tail coverage (LTC). In this case, we calculate the percentage of long-tail items that are appeared in recommendation lists. Thus, we need to determine the long-tail items from training data. To do this, we create cumulative popularity list of items sorted from most popular to less-popular items, then we define a cutting point such that it divides the items into short-head and long-tail items. 
%For experiments in this paper, we used cutting point of 20\%, meaning that 20\% of most popular items are considered as short-head items and the rest of less popular items are considered as long-tail items. 

Figure \ref{fig2} shows the performance of two recommendation algorithms on four data sets and different input values in terms of item coverage and nDCG.

\begin{figure*}[!tbp]
  \begin{subfigure}[b]{0.8\textwidth}
    \includegraphics[width=\textwidth]{bx.png}
    \caption{Bookcrossing}
    \label{fig:f1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.8\textwidth}
    \includegraphics[width=\textwidth]{cio.png}
    \caption{CiaoDVD}
    \label{fig:f2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.8\textwidth}
    \includegraphics[width=\textwidth]{ft.png}
    \caption{FilmTrust}
    \label{fig:f2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.8\textwidth}
    \includegraphics[width=\textwidth]{ml1m.png}
    \caption{MovieLens1M}
    \label{fig:f2}
  \end{subfigure}
  \hfill
  %\begin{subfigure}[b]{0.33\textwidth}
  %  \includegraphics[width=\textwidth]{rate-userknn-log.png}
  %  \caption{UserKNN}
  %  \label{fig:f2}
  %\end{subfigure}
  \caption{Item coverage versus nDCG@10 for two recommendation algorithms on different data sets. Plots on right side are results of SVD++ and plots on left side are results of Biased Matrix Factorization.} \label{fig2}
\end{figure*}

Another methodology for analyzing item popularity has been proposed in \cite{Cremonesi:2010a}. In this methodology, accuracy of recommendation algorithms on long-tail items is considered. The main goal was measuring the effectiveness of a recommendation algorithm on how accurate it can recommend long-tail items.

Table \ref{tab:reslongtail} shows the performance of recommendation algorithms on long-tail items. 

\input{ndcg_longtail_table.tex}

%\subsection{Flatness analysis} \label{flatanalysis}

%We hypothesize that a transformation that produces a flatter distribution will compensate for skew and variance in rating distributions and generate improved recommendation performance. As we have seen, the percentile transformation generally leads to better performance and to flatter distributions, and the less-flat z-score transformation has lower performance.

%We examined this phenomena using three types of inputs for recommender system: original ratings, percentile values, and z-score values.\footnote{Because a limitation in LibRec, z-score values are shifted to positive values by the addition of an offset value.} We used three of the sparser data sets and examined the $\mathcal{F}$ value for the ratings under the different transformations and the recommendation performance using nDCG@10. The data set is divided into train and test sets as 80\% and 20\%, respectively, and $\mathcal{F}$ value is calculated on the training set.  

%For this exploration, we used three latent-factor algorithms: \algname{BiasedMF}, \algname{ListRank}, and \algname{SVD++}. To be comparable, parameter values for these algorithms were assigned in a uniform manner. For the BX and Yelp data set, the number of factors and the number of iterations are set to 100 and 20 over all algorithms, respectively, and on CiaoDVD data set, the number of factors and the number of iterations are set to 150 and 20 over all algorithms, respectively. We conducted experiments with different number of factors and iterations and we observed that over most of the settings, the results support our hypothesis.

%Figure~\ref{fig:flatness} clearly shows the negative correlation between performance and divergence from flatness. (Note that a low $\mathcal{F}$ value corresponds to a flatter distribution.) The flatter distributions (closer to zero) yield better performance for all three algorithms across all data sets. Table \ref{tab:cor} shows the correlation between $\mathcal{F}$ value of each input values (i.e., original ratings, percentile values, and z-score values) and nDCG@10 of recommendation algorithms with those input values. Correlation value of -0.97 obtained from \algname{BiasedMF} on BX, for instance, is calculated between the $\mathcal{F}$ values of 0.1006, 0.4494, 0.6976 and nDCG@10 values of 0.0076, 0.0035, 0.0026 resulted from percentile values, original ratings, and z-score values, respectively. As shown in Table \ref{tab:cor}, the observed correlations between $\mathcal{F}$ and nDCG are between -0.99 and -0.81 for all the algorithms and all data sets, indicative of a strong inverse relationship.

%\input{fig2}
%\begin{figure} 
%\includegraphics[height=2in, width=5in]{bx.png}
%\caption{}\label{fig1}
%\end{figure}





%\input{coverage_table1.tex}
%\input{coverage_table2.tex}
%\input{coverage_table4.tex}
%\input{coverage_table5.tex}

\section{Conclusions}



==> conf.tex <==
\captionsetup[table]{skip=4pt}
\begin{table}[t!]
\small
\centering
\captionof{table}{Parameters configuration for results reported in table \ref{tab:res1}} \label{tab:conf}
\begin{tabular}{lrrrrrrrr}
\toprule
 %\multirow{2}{*}{Dataset} &  &  &  &  &  & \multicolumn{3}{c}{Smoothed percentile} \\ \cline{7-9}
  %& rating & z-score & $\mbox{Per}^f_u$ & $\mbox{Per}^m_u$ & $\mbox{Per}^l_u$ & $\mbox{Per}^f_u$ & $\mbox{Per}^m_u$ & $\mbox{Per}^l_u$ \\
 dataset & algorithm & z-score & $\mbox{Per}^f_u$ & $\mbox{Per}^m_u$ & $\mbox{Per}^l_u$ & $\mbox{SPer}^f_u$ & $\mbox{SPer}^m_u$ & $\mbox{SPer}^l_u$ \\
 \midrule
 MovieLens1M & 0.154 & 0.593 &  && \bf{0.134} &  && \\
 Yelp & 0.205 & 0.422 &  && \bf{0.137} &&& \\
 CiaoDVD & 0.314 & 0.371 &  && \bf{0.153} &&& \\
 BX & 0.448 & 0.582 &  && \bf{0.1} &&& \\
\bottomrule
\multicolumn{4}{l}{\textit{Flatness of a uniform distribution is $\mathcal{F}=0$.}} \\
\end{tabular}
\end{table}


==> ndcg_longtail_smoothed_table.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms on long-tail items at nDCG@10 } \label{tab:reslongtail}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{dataset} & \multirow{2}{*}{algorithms} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & $zscore_u$ & $first_u$ & $ceil_u$ & $last_u$ & & $first_u$ & $ceil_u$ & $last_u$ \\
 \bottomrule
 
 
% rate => biasedmf-user-u0.005-i0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0                
% zscore => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.005-fac100-20.0
% first,ceil,last => iasedmf-user-u0.005-i0.005-bias0.005-itemax100-itelearn0.005-fac150-20.0
% smoothed first,ceil => biasedmf-user-u0.01-i0.01-bias0.01-itemax100-itelearn0.01-fac150-20.0
% smoothed last => biasedmf-user-u0.01-i0.01-bias0.01-itemax100-itelearn0.005-fac150-20.0
 \multirow{2}{*}{BX} & \algname{BiasedMF} & 0.0008 & 0.0009 & \bf{0.0018} & \bf{0019} & \bf{0034} & & \bf{0.0048} & \bf{0.0045} & \bf{0.0044} \\
% rate => svdpp-user--u0.01-i0.01-impItem0.01-bias0.01-itemax100-itelearn0.01-fac150-20.0
% zscore => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.001-fac100-20.0
% first => svdpp-user--u0.01-i0.01-impItem0.01-bias0.01-itemax50-itelearn0.005-fac150-20.0
% ceil  => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.005-fac150-20.0
% last  => svdpp-user--u0.01-i0.01-impItem0.01-bias0.01-itemax100-itelearn0.005-fac150-20.0
% smoothe all => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.005-fac150-20.0      
 & \algname{SVD++} & 0.0011 & 0.0009 & \bf{0.0024} & \bf{0.0024} & \bf{0.0043} & & \bf{0.0048} & \bf{0.0047} & \bf{0.0046} \\


\cline{1-11}


% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.001-fac50-20.0
% first,last => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac50-20.0
% ceil => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac100-20.0
% smoothed all => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
 \multirow{2}{*}{CiaoDVD} & \algname{BiasedMF} & 0.019 & 0.005 & \bf{0.027} & \bf{0.024} & 0.016 & & \bf{0.027} & \bf{0.027} & \bf{0.026} \\
% rate => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.001-fac50-20.0
% zscore => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax50-itelearn0.005-fac100-20.0
% first,ceil => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.0001-fac50-20.0
% last => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
 & \algname{SVD++} & 0.009 & 0.011 & \bf{0.022} & \bf{0.019} & \bf{0.017} & & \bf{0.019} & \bf{0.018} & \bf{0.016} \\


 \cline{1-11}


%rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.005-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% first,ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac150-20.0
% smoothed first,ceil -> biasedmf-user-u0.01-i0.01-bias0.01-itemax100-itelearn0.0001-fac50-20.0
% smoothed last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
 \multirow{2}{*}{FilmTrust} & \algname{BiasedMF} & 0.0581 & 0.0667 & \bf{0.1991} & \bf{0.2109} & \bf{0.2268} & & \bf{0.2110} & \bf{0.2185} & \bf{0.2142} \\
% rate => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% zscore => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% first => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax50-itelearn0.001-fac50-20.0
% ceil,last  => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
% smoothed => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
 & \algname{SVD++} & 0.0279 & 0.072 & \bf{0.0603} & \bf{0.0696} & \bf{0.1006} & & \bf{0.0620} & \bf{0.0740} & \bf{0.0851} \\


\cline{1-11}


% rate   => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.005-fac100-20.0
% zscore => biasedmf-user-u0.01-i0.01-bias0.01-itemax30-itelearn0.005-fac100-20.0
% first => biasedmf-user-u0.01-i0.01-bias0.01-itemax50-itelearn0.0001-fac100-20.0
% ceil  => biasedmf-user-u0.01-i0.01-bias0.01-itemax100-itelearn0.0001-fac50-20.0
% last  => biasedmf-user-u0.005-i0.005-bias0.005-itemax50-itelearn0.0001-fac100-20.0
% smoothed first,ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% smoothed last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
 \multirow{2}{*}{ML1M} & \algname{BiasedMF} & 0.0364 & 0.0360 & 0.0359 & \bf{0.0379} & \bf{0.0389} & & \bf{0.0374} & \bf{0.0390} & \bf{0.0394} \\
% rate,zscore => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.001-fac50-20.0
% first=> svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% ceil,last => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
% smoothed => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
 & \algname{SVD++} & 0.0461 & 0.0461 & 0.0426 & \bf{0.0471} & \bf{0.0497} & & \bf{0.0490} & \bf{0.0529} & \bf{0.0533} \\

 
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/coverage_table1.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms in terms of item coverage on BX dataset } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{metrics} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & zscore & first & ceil & last & & first & ceil & last \\
 \bottomrule
%  \multirow{3}{*}{\algname{UserKNN}} 
%  & $CC_u$         & 52.18\% & 52.90\% & 52.87\% & 52.66\% & \bf{53.14}\% & &  &  &  \\
%  & $LTC_u$        & 50.62\% & 51.36\% & 51.33\% & 51.11\% & \bf{51.60}\% & &  &  &  \\
%  & $CC_i$         &  & \color{red}\bf{56.67}\% & 56.37\% & 56.37\% & 56.13\% & &  &  &  \\
%  & $LTC_i$        &  & \color{red}\bf{55.25}\% & 54.94\% & 54.94\% & 54.70\% & &  &  &  \\
% rate => userknn-user-usersim-pcc-shrink0-knn30-20.0
% zscore,first,ceil,last => userknn-user-usersim-pcc-shrink10-knn30-20.0
%  & $CC_{ubest}$   & 52.77\% & 53.27\% & \bf{53.37}\% & 53.15\% & \bf{53.69}\% & &  &  &  \\
%  & $LTC_{ubest}$  & 51.22\% & 51.74\% & \bf{51.85}\% & 51.62\% & \bf{52.18}\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.013 & 0.014 & 0.014 & 0.014 & 0.014 & &  &  &  \\
% zscore,first,ceil.last => userknn-item-usersim-pcc-shrink10-knn200-20.0
%  & $CC_{ibest}$   &  & \color{red}\bf{57.73}\% & 57.37\% & 57.50\% & 57.29\% & &  &  &  \\
%  & $LTC_{ibest}$  &  & \color{red}\bf{56.34}\% & 55.97\% & 56.10\% & 55.89\% & &  &  &  \\
%  & $nDCG_{ibest}$ &  & 0.026 & 0.026 & 0.026 & 0.025 & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{ItemKNN}} 
%  & $CC_u$         & 24.35\% & 24.52\% & \bf{25.61\%} & \bf{25.16\%} & \bf{25.01\%} & &  &  &  \\
%  & $LTC_u$        & 21.9 & 22.08\% & \bf{23.19\%} & \bf{22.73\%} & \bf{22.59\%} & &  &  &  \\
%  & $CC_i$         & 24.35\% & 24.72\% & \bf{25.43}\% & \bf{25.24}\% & \bf{25.10}\% & & \bf{25.24}\% & \bf{25.20}\% & \bf{25.11}\% \\
%  & $LTC_i$        & 21.91\% & 22.28\% & \bf{23.02}\% & \bf{22.81}\% & \bf{22.66}\% & & \bf{22.83}\% & \bf{22.78}\% & \bf{22.69}\% \\
% rate => itemknn-item-itemsim-cos-shrink0-knn10-20.0
% all => itemknn-user-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ubest}$   & 40.67\% & \color{red}\bf{42.85\%} & 42.46\% & 42.69\% & 42.49\% & &  &  &  \\
%  & $LTC_{ubest}$  & 38.72\% & \color{red}\bf{40.98\%} & 40.57\% & 40.81\% & 40.61\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.009 & 0.009 & 0.009 & 0.009 & 0.009 & &  &  &  \\
% zscore,smoothed => itemknn-item-itemsim-cos-shrink0-knn10-20.0
% first,ceil,last => itemknn-item-itemsim-cos-shrink0-knn20-20.0
%  & $CC_{ibest}$   &  & 43.60\% & 41.85\% & 41.80\% & 41.90\% & & 43.54\% & \bf{44.21}\% & 43.31\% \\
%  & $LTC_{ibest}$  &  & 41.76\% & 39.94\% & 39.90\% & 40.00\% & & 41.69\% & \bf{42.39}\% & 41.46\% \\
%  & $nDCG_{ibest}$ &  & 0.009 & \bf{0.012} & \bf{0.012} & \bf{0.013} & & 0.009 & 0.009 & 0.009 \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{SLIM}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{BiasedMF}} 
%  & $CC_u$         &  &  &  &  &  & & 0.31\% & 0.31\% & 0.32\% \\
%  & $LTC_u$        &  &  &  &  &  & & 0.06\% & 0.07\% & 0.08\% \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% zscore => biasedmf-item-u0.005-i0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% first,ceil,last => biasedmf-item-u0.01-i0.01-bias0.01-itemax100-itelearn0.005-fac150-20.0
% smoothed => biasedmf-item-u0.01-i0.01-bias0.01-itemax100-itelearn0.005-fac150-20.0
  & $CC_{ibest}$   & 34.49\% & 54.67\% & 52.29\% & 53.43\% & 41.73\% & & 57.76\% & 53.38\% & 45.57\% \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ & 0.003 & 0.001 & 0.007 & 0.008 & 0.010 & & 0.006 & 0.007 & 0.009 \\
  
 \cline{1-11}
 
% \multirow{3}{*}{\algname{ListRank}} 
%  & $CC_u$         & 5.22\% & 0.20\% & \bf{33.92}\% & \bf{34.55}\% & \bf{34.03}\% & &  &  &  \\
%  & $LTC_u$        & 3.32\% & 0.00\% & \bf{31.76}\% & \bf{32.41}\% & \bf{31.87}\% & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% rate,zscore,ceil,last => listrankmf-user-u0.005-i0.005-itemax100-itelearn0.001-fac150-20.0
% first => listrankmf-user-u0.001-i0.001-itemax100-itelearn0.01-fac150-20.0
%  & $CC_{ubest}$   & 36.47\% & 27.98\% & \bf{41.92}\% & \bf{40.49}\% & \bf{39.94}\% & &  &  &  \\
%  & $LTC_{ubest}$  & 34.41\% & 25.64\% & \bf{40.02}\% & \bf{38.55}\% & \bf{37.97}\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.011 & 0.012 & 0.007 & 0.011 & 0.012 & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{SVD++}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
% rate => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% zscore => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.001-fac150-20.0
% first,last => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.005-fac150-20.0
% ceil => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% smoothed => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.005-fac150-20.0
  & $CC_{ibest}$   & 55.50\% & 71.00\% & 50.19\% & 58.24\% & 39.44\% & & 51.77\% & 48.28\% & 42.32\% \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ & 0.002 & 0.001 & 0.007 & 0.004 & 0.010 & & 0.006 & 0.007 & 0.009 \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{NMF}}
%  & $CC_u$         & 18.01\% & \color{red}\bf{24.02}\% & 12.37\% & 19.66\% & 22.97\% & & 11.80\% & 15.44\% & 17.59\% \\
%  & $LTC_u$        & 17.63\% & \color{red}\bf{24.12}\% & 12.41\% & 18.98\% & 22.12\% & & 11.82\% & 15.35\% & 17.06\% \\
%  & $CC_i$         &  & 13.66\% & 12.03\% & \bf{14.24}\% & \bf{16.42}\% & & \bf{15.68}\% & \bf{16.21}\% & \bf{17.10}\% \\
%  & $LTC_i$        &  & 14.08\% & 11.89\% & 13.79\% & \bf{15.62}\% & & \bf{15.38}\% & \bf{15.80}\% & \bf{16.29}\% \\
% rate => nmf-user--itemax100-fac50-20.0
% zscore => nmf-user--itemax100-fac50-20.0
% first,ceil,last => nmf-user--itemax50-fac100-20.0
% smoothed first => nmf-user--itemax100-fac100-20.0
% smoothed ceil,last => nmf-user--itemax50-fac50-20.0
%  & $CC_{ubest}$   & 20.75\% & \color{red}\bf{24.02}\% & 15.90\% & 19.67\% & 23.18\% & & 12.38\% & 15.68\% & 18.35\% \\
%  & $LTC_{ubest}$  & 20.60\% & \color{red}\bf{24.12}\% & 15.60\% & 19.29\% & 22.73\% & & 12.18\% & 15.90\% & 18.56\% \\
%  & $nDCG_{ubest}$ & 0.0004 & 0.0004 & 0.0004 & 0.0006 & 0.0006 & & 0.0004 & 0.0005 & 0.0005 \\
% first => nmf-item--itemax30-fac100-20.0
% ceil,last => nmf-item--itemax50-fac150-20.0
% zscore => nmf-item--itemax100-fac50-20.0
% smoothed first => nmf-item--itemax50-fac50-20.0
% smoothed ceil,last => nmf-item--itemax100-fac50-20.0
%  & $CC_{ibest}$   &  & \color{red}\bf{22.95}\% & 12.60\% & 14.27\% & 16.45\% & & 15.79\% & 16.70\% & 17.50\% \\
%  & $LTC_{ibest}$  &  & \color{red}\bf{23.19}\% & 12.79\% & 14.10\% & 16.05\% & & 16.06\% & 16.54\% & 16.99\% \\
%  & $nDCG_{ibest}$ &  & 0.0005 & \bf{0.0006} & \bf{0.0006} & \bf{0.0006} & & 0.0004 & 0.0004 & 0.0005 \\
  
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/coverage_table2.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms in terms of item coverage on CiaoDVD dataset } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{metrics} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & zscore & first & ceil & last & & first & ceil & last \\
 \bottomrule
%  \multirow{3}{*}{\algname{UserKNN}} 
%  & $CC_u$         & 17.04\% & 17.32\% & 17.24\% & 17.28\% & \bf{17.33\%} & & \bf{17.37\%} & \bf{17.35\%} & \bf{17.40\%} \\
%  & $LTC_u$        & 16.15\% & 16.42\% & 16.34\% & 16.39\% & \bf{16.44\%} & & \bf{16.48\%} & \bf{16.46\%} & \bf{16.51\%} \\
%  & $CC_i$         &  & \color{red}\bf{21.46\%} & 20.98\% & 21.28\% & 21.28\% & & 20.79\% & 21.10\% & 21.08\% \\
%  & $LTC_i$        &  & \color{red}\bf{20.60\%} & 20.12\% & 20.43\% & 20.43\% & & 19.93\% & 20.24\% & 20.22\% \\
% all => userknn-user-usersim-pcc-shrink0-knn20-20.0
% smoothed => userknn-user-usersim-pcc-shrink0-knn20-20.0
%  & $CC_{ubest}$   & 17.33\% & 17.54\% & 17.54\% & \bf{17.57\%} & \bf{17.55\%} & & \bf{17.65\%} & \bf{17.58\%} & \bf{17.57\%} \\
%  & $LTC_{ubest}$  & 16.44\% & 16.65\% & 16.65\% & \bf{16.67\%} & \bf{16.66\%} & & \bf{16.76\%} & \bf{16.69\%} & \bf{16.68\%} \\
%  & $nDCG_{ubest}$ & 0.009 & 0.009 & 0.009 & 0.009 & 0.009 & & 0.009 & 0.009 & 0.009 \\
% all => userknn-item-usersim-pcc-shrink0-knn40-20.0
% zscore => userknn-item-usersim-pcc-shrink20-knn70-20.0
% smoothed => userknn-item-usersim-pcc-shrink0-knn40-20.0
%  & $CC_{ibest}$   &  & \color{red}\bf{21.62\%} & 21.25\% & 21.43\% & 21.52\% & & 21.08\% & 21.35\% & 21.33\% \\
%  & $LTC_{ibest}$  &  & \color{red}\bf{20.69\%} & 20.39\% & 20.57\% & 20.66\% & & 20.23\% & 20.49\% & 20.47\% \\
%  & $nDCG_{ibest}$ &  & 0.009 & 0.010 & 0.009 & 0.010 & & 0.010 & 0.010 & 0.010 \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{ItemKNN}} 
%  & $CC_u$         & 35.19\% & \color{red}\bf{37.96\%} & 37.51\% & 37.23\% & 37.19\% & & 37.87\% & 37.95\% & 37.78\% \\
%  & $LTC_u$        & 34.49\% & \color{red}\bf{37.29\%} & 36.84\% & 36.55\% & 36.51\% & & 37.19\% & 37.28\% & 37.11\% \\
%  & $CC_i$         &  & 37.90\% & 36.54\% & 36.28\% & 36.21\% & & \bf{41.24\%} & \bf{38.46\%} & \bf{41.41\%} \\
%  & $LTC_i$        &  & 37.23\% & 35.85\% & 35.59\% & 35.52\% & & \bf{40.60\%} & \bf{37.79\%} & \bf{40.77\%} \\
% rate => itemknn-item-itemsim-cos-shrink0-knn10-20.0
% zscore,first,ceil,last,smoothed => itemknn-user-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ubest}$   & 36.03\% & \color{red}\bf{41.08\%} & 39.45\% & 39.41\% & 39.39\% & & 40.64\% & 40.95\% & 40.75\% \\
%  & $LTC_{ubest}$  & 35.33\% & \color{red}\bf{40.44\%} & 38.79\% & 38.75\% & 38.73\% & & 40.00\% & 40.31\% & 40.10\% \\
%  & $nDCG_{ubest}$ & 0.006 & 0.005 & 0.005 & 0.005 & 0.005 & & 0.006 & 0.006 & 0.005 \\
% all,smoothed => itemknn-item-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ibest}$   &  & 40.99\% & 38.66\% & 38.43\% & 38.78\% & & \bf{45.65\%} & \bf{42.16\%} & \bf{46.29\%} \\
%  & $LTC_{ibest}$  &  & 40.35\% & 38.00\% & 37.76\% & 38.11\% & & \bf{45.06\%} & \bf{41.53\%} & \bf{45.70\%} \\
%  & $nDCG_{ibest}$ &  & 0.005 & 0.006 & 0.006 & 0.006 & & 0.005 & 0.005 & 0.005 \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{SLIM}} 
%  & $CC_u$         & 60.39\% & \color{red}\bf{63.78\%} & 61.56\% & 60.01\% & 63.27\% & & 48.11\% & 60.97\% & 63.73\% \\
%  & $LTC_u$        & 59.97\% & \color{red}\bf{63.40\%} & 61.25\% & 59.68\% & 62.88\% & & 47.60\% & 60.59\% & 63.36\% \\
%  & $CC_i$         &  & 60.26\% & 60.77\% & 60.11\% & 59.21\% & & \bf{64.49\%} & \bf{62.24}\% & \bf{63.64\%} \\
%  & $LTC_i$        &  & 59.83\% & 60.37\% & 59.69\% & 58.79\% & & \bf{64.14\%} & \bf{61.84\%} & \bf{63.26\%} \\
% rate => slim-item-itemsim-cos-knn100-itemax30-l10.05-l25-20.0
%zscore => slim-user-itemsim-cos-knn100-itemax50-l10.05-l25-20.0
% first,ceil,last => slim-user-itemsim-cos-knn100-itemax30-l10.05-l22-20.0
% smoothed => slim-user-itemsim-cos-knn100-itemax30-l10.05-l20.5-20.0
%  & $CC_{ubest}$   & 62.37\% & \color{red}\bf{64.97\%} & 63.84\% & 63.89\% & 63.37\% & & 63.86\% & 64.46\% & 64.04\% \\
%  & $LTC_{ubest}$  & 61.97\% & \color{red}\bf{64.60\%} & 63.50\% & 63.57\% & 63.05\% & & 63.50\% & 64.10\% & 63.70\% \\
%  & $nDCG_{ubest}$ & 0.005 & 0.005 & 0.003 & 0.002 & 0.002 & & 0.003 & 0.003 & 0.002 \\
% zscore => slim-item-itemsim-cos-knn100-itemax30-l10.05-l25-20.0
% first => slim-item-itemsim-cos-knn100-itemax50-l10.05-l25-20.0
% ceil => slim-item-itemsim-cos-knn100-itemax100-l10.05-l20.5-20.0
% last => slim-item-itemsim-cos-knn100-itemax30-l10.05-l20.05-20.0
% smoothed => slim-item-itemsim-cos-knn50-itemax50-l10.5-l22-20.0
%  & $CC_{ibest}$   &  & 61.28\% & 63.24\% & 61.96\% & 60.32\% & & \bf{65.03\%} & 62.46\% & \bf{63.84\%} \\
%  & $LTC_{ibest}$  &  & 60.86\% & 62.86\% & 61.56\% & 59.90\% & & \bf{64.68\%} & 62.07\% & \bf{63.47\%} \\
%  & $nDCG_{ibest}$ &  & 0.005 & 0.003 & 0.003 & 0.003 & & 0.003 & 0.003 & 0.003 \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{BiasedMF}} 
%  & $CC_u$         & 4.85\% & 6.82\% & 0.15\% & 0.22\% & 0.21\% & & 0.13\% & 0.15\% & 0.18\% \\
%  & $LTC_u$        & 4.02\% & 5.88\% & 0.01\% & 0.02\% & 0.04\% & & 0\% & 0\% & 0\% \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
% rate => biasedmf-user-u0.01-i0.01-bias0.01-itemax30-itelearn0.0001-fac150-20.0
% zscore => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.001-fac150-20.0
% first,ceil => biasedmf-item-u0.01-i0.01-bias0.01-itemax30-itelearn0.0001-fac150-20.0
% last => biasedmf-item-u0.01-i0.01-bias0.01-itemax100-itelearn0.005-fac100-20.0
% smoothed first => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.01-fac150-20.0
% smoothed ceil => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.005-fac150-20.0
% smoothed last => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac150-20.0
  & $CC_{ibest}$   & 42.84\% & 52.52\% & 42.84\% & 39.44\% & 9.82\% & & 39.80\% & 31.49\% & 11.72\% \\
%  & $LTC_{ibest}$  & 37.91\% & 46.75\% & 37.91\% & 15.58\% & 8.84\% & &  &  &  \\
  & $nDCG_{ibest}$ & 0.001 & 0.002 & 0.001 & 0.002 & 0.004 & & 0.002 & 0.004 & 0.009 \\
  
 \cline{1-11}
 
% \multirow{3}{*}{\algname{ListRank}} 
%  & $CC_u$         & 1.59\% & 0.18\% & 2.48\% & 1.83\% & 1.72\% & & 5.28\% & 5.27\% & 5.17\% \\
%  & $LTC_u$        & 1.23\% & 0.04\% & 1.95\% & 1.48\% & 1.37\% & & 4.33\% & 4.31\% & 4.23\% \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% smoothed all => listrankmf-user-u0.005-i0.005-itemax100-itelearn0.0001-fac150-20.0
%  & $CC_{ubest}$   &  &  &  &  &  & & 12.89\% & 12.48\% & 12.53\% \\
%  & $LTC_{ubest}$  &  &  &  &  &  & & 11.94\% & 11.53\% & 11.58\% \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & & 0.010 & 0.010 & 0.010 \\
% zscore => listrankmf-item-u0.001-i0.001-itemax100-itelearn0.0001-fac150-20.0
% first => listrankmf-item-u0.01-i0.01-itemax100-itelearn0.0001-fac150-20.0
% ceil => listrankmf-item-u0.01-i0.01-itemax100-itelearn0.005-fac150-20.0
% last => listrankmf-item-u0.01-i0.01-itemax100-itelearn0.0001-fac150-20.0
%  & $CC_{ibest}$   &  & 8.64\% & 9.98\% & 12.39\% & 11.58\% & &  &  &  \\
%  & $LTC_{ibest}$  &  & 7.65\% & 9.01\% & 11.44\% & 10.62\% & &  &  &  \\
%  & $nDCG_{ibest}$ &  & 0.014 & 0.009 & 0.010 & 0.009 & &  &  &  \\
  
 \cline{1-11}
 
 \multirow{3}{*}{\algname{SVD++}} 
%  & $CC_u$         & 6.19\% & 15.04\% & 0.45\% & 0.28\% & 4.98\% & &  &  &  \\
%  & $LTC_u$        & 5.30\% & 13.80\% & 0.13\% & 0.06\% & 3.96\% & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
% rate => svdpp-user--u0.001-i0.001-impItem0.001-bias0.001-itemax30-itelearn0.0001-fac150-20.0
% zscore => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.001-fac150-20.0
% first,ceil => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% last => svdpp-item--u0.01-i0.01-impItem0.01-bias0.01-itemax100-itelearn0.005-fac150-20.0
% smoothed => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.005-fac150-20.0
  & $CC_{ibest}$   & 65.28\% & 70.99\% & 34.54\% & 63.54\% & 13.78\% & & 39.99\% & 36.32\% & 20.80\% \\
%  & $LTC_{ibest}$  &  & 63.13\% & 32.23\% & 56.80\% & 12.85\% & &  &  &  \\
  & $nDCG_{ibest}$ & 0.0006 & 0.0004 & 0.006 & 0.001 & 0.009 & & 0.004 & 0.005 & 0.009 \\
  
% \cline{1-11}
 
%  \multirow{3}{*}{\algname{SVD++}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
 
 
% \multirow{3}{*}{\algname{NMF}}
%  & $CC_u$         & 1.06\% & 2.42\% & \bf{2.59}\% & \bf{4.00}\% & \bf{4.21}\% & &  &  &  \\
%  & $LTC_u$        & 1.06\% & 2.45\% & \bf{2.58}\% & \bf{3.98}\% & \bf{4.16}\% & &  &  &  \\
%  & $CC_i$         &  & 2.14\% & \bf{2.97}\% & 2.92\% & 2.75\% & & 1.56\% & 1.33\% & 1.29\% \\
%  & $LTC_i$        &  & 2.17\% & \bf{3.00}\% & 2.95\% & 2.77\% & & 1.57\% & 1.34\% & 1.29\% \\
% rate => nmf-item--itemax100-fac50-20.0
% zscore,first,ceil,last => nmf-user--itemax100-fac50-20.0  
%  & $CC_{ubest}$   & 1.93\% & 3.87\% & 2.59\% & \bf{4.00}\% & \bf{4.21}\% & &  &  &  \\
%  & $LTC_{ubest}$  & 1.94\% & 3.90\% & 2.58\% & \bf{3.98}\% & \bf{4.16}\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.0001 & 0.00004 & 0.0001 & 0.0001 & 0.0001 & &  &  &  \\
% first => nmf-item--itemax30-fac50-20.0
% ceil => nmf-item--itemax50-fac50-20.0
% last,zscore => nmf-item--itemax100-fac50-20.0
% smoothed first => nmf-item--itemax50-fac50-20.0
% smoothed ceil,last => nmf-item--itemax100-fac50-20.0
%  & $CC_{ibest}$   &  & \color{red}\bf{4.19}\% & 2.97\% & 3.02\% & 2.90\% & & 2.28\% & 2.10\% & 2.13\% \\
%  & $LTC_{ibest}$  &  & \color{red}\bf{4.22}\% & 3.00\% & 3.04\% & 2.86\% & & 2.30\% & 2.10\% & 2.10\% \\
%  & $nDCG_{ibest}$ &  & 0.0001 & 0.0001 & 0.0001 & 0.0001 & & 0.0001 & 0.0001 & 0.0001 \\
  
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/coverage_table3.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms in terms of item coverage on Epinions dataset } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{metrics} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & zscore & first & ceil & last & & first & ceil & last \\
 \bottomrule
%  \multirow{3}{*}{\algname{UserKNN}} 
%  & $CC_u$         & 5.95\% & 5.75\% & 6.11\% & 5.91\% & 5.98\% & & 43.50\% & 43.48\% & 43.38\% \\
%  & $LTC_u$        & 3.33\% & 3.16\% & 3.58\% & 3.40\% & 3.41\% & & 41.60\% & 41.57\% & 41.47\% \\
%  & $CC_i$         &  & 5.71\% & 6.12\% & 5.99\% & 5.95\% & &  &  &  \\
%  & $LTC_i$        &  & 3.14\% & 3.51\% & 3.36\% & 3.30\% & &  &  &  \\
% rate => itemknn-item-itemsim-cos-shrink0-knn10-20.0
% zscore,first,ceil,last => itemknn-user-itemsim-cos-shrink0-knn10-20.0
% smoothed => userknn-user-usersim-pcc-shrink20-knn100-20.0
%  & $CC_{ubest}$   & 78.26\% & 82.21\% & 82.16\% & 82.09\% & 81.87\% & & 47.04\% & 46.93\% & 46.92\% \\
%  & $LTC_{ubest}$  & 77.52\% & 81.61\% & 81.56\% & 81.48\% & 81.25\% & & 45.25\% & 45.14\% & 45.13\% \\
%  & $nDCG_{ubest}$ & 0.005 & 0.005 & 0.004 & 0.004 & 0.004 & & 0.063 & 0.063 & 0.063 \\
% all => itemknn-item-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ibest}$   &  & 82.56\% & 81.82\% & 82.45\% & 82.53\% & &  &  &  \\
%  & $LTC_{ibest}$  &  & 81.97\% & 81.21\% & 81.86\% & 81.94\% & &  &  &  \\
%  & $nDCG_{ibest}$ &  & 0.004 & 0.005 & 0.005 & 0.005 & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{ItemKNN}} 
%  & $CC_u$         & 5.95\% & 5.75\% & 6.11\% & 5.91\% & 5.98\% & &  &  &  \\
%  & $LTC_u$        & 3.33\% & 3.16\% & 3.58\% & 3.40\% & 3.41\% & &  &  &  \\
%  & $CC_i$         &  & 5.71\% & 6.12\% & 5.99\% & 5.95\% & & 6.31\% & 6.75\% & 6.55\% \\
%  & $LTC_i$        &  & 3.14\% & 3.51\% & 3.36\% & 3.30\% & & 3.69\% & 4.04\% & 3.85\% \\
% rate => itemknn-item-itemsim-cos-shrink0-knn10-20.0     
% zscore,first,ceil,last => itemknn-user-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ubest}$   & 78.26\% & 82.21\% & 82.16\% & 82.09\% & 81.87\% & &  &  &  \\
%  & $LTC_{ubest}$  & 77.52\% & 81.61\% & 81.56\% & 81.48\% & 81.25\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.005 & 0.005 & 0.004 & 0.004 & 0.004 & &  &  &  \\
% all => itemknn-item-itemsim-cos-shrink0-knn10-20.0
% smoothed => itemknn-item-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ibest}$   &  & 82.56\% & 81.82\% & 82.45\% & 82.53\% & & 82.23\% & 82.80\% & 83.11\% \\
%  & $LTC_{ibest}$  &  & 81.97\% & 81.21\% & 81.86\% & 81.94\% & & 81.63\% & 82.22\% & 82.54\% \\
%  & $nDCG_{ibest}$ &  & 0.004 & 0.005 & 0.005 & 0.005 & & 0.005 & 0.005 & 0.005 \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{SLIM}} 
%  & $CC_u$         & 84.73\% & \color{red}\bf{96.22\%} & 88.13\% & 90.20\% & 91.32\% & & 90.05\% & 91.34\% & 92.25\% \\
%  & $LTC_u$        & 84.47\% & \color{red}\bf{96.09\%} & 87.81\% & 89.94\% & 91.09\% & & 89.78\% & 91.13\% & 92.03\% \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% all => slim-user-itemsim-cos-knn100-itemax30-l10.05-l20.05-20.0
% smoothed => slim-user-itemsim-cos-knn100-itemax30-l10.05-l20.05-20.0
%  & $CC_{ubest}$   & 85.03\% & \color{red}\bf{96.17\%} & 88.15\% & 90.20\% & 91.54\% & & 90.33\% & 91.46\% & 92.33\% \\
%  & $LTC_{ubest}$  & 84.74\% & \color{red}\bf{96.04\%} & 87.83\% & 89.93\% & 91.32\% & & 90.07\% & 91.26\% & 92.12\% \\
%  & $nDCG_{ubest}$ & 0.010 & 0.009 & 0.007 & 0.008 & 0.008 & & 0.008 & 0.008 & 0.008 \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{BiasedMF}} 
  & $CC_u$         &  &  &  &  &  & &  &  &  \\
  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
  & $CC_i$         &  &  &  &  &  & &  &  &  \\
  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
 \cline{1-11}
 
% \multirow{3}{*}{\algname{ListRank}} 
%  & $CC_u$         & 8.06\% & 0.58\% & 6.76\% & 10.33\% &  & &  &  &  \\
%  & $LTC_u$        & 5.42\% & 0.08\% & 4.28\% & 7.47\% &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% rate => listrankmf-user-u0.001-i0.001-itemax100-itelearn0.01-fac100-20.0
% zscore => listrankmf-user-u0.005-i0.005-itemax100-itelearn0.005-fac150-20.0
% first => listrankmf-user-u0.001-i0.001-itemax100-itelearn0.01-fac150-20.0
% ceil => listrankmf-user-u0.001-i0.001-itemax100-itelearn0.01-fac100-20.0
% last => listrankmf-user-u0.001-i0.001-itemax100-itelearn0.001-fac100-20.0
%  & $CC_{ubest}$   & 39.62\% & 21.03\% & 32.47\% & 44.95\% & 47.32\% & &  &  &  \\
%  & $LTC_{ubest}$  & 37.59\% & 18.37\% & 30.24\% & 43.10\% & 45.54\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.017 & 0.015 & 0.011 & 0.014 & 0.011 & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{SVD++}} 
  & $CC_u$         &  &  &  &  &  & &  &  &  \\
  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
  & $CC_i$         &  &  &  &  &  & &  &  &  \\
  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{NMF}}
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/coverage_table4.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms in terms of item coverage on FilmTrust dataset } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{metrics} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & zscore & first & ceil & last & & first & ceil & last \\
 \bottomrule
 
 % rate,zscore,ceil,last => userknn-user-usersim-pcc-shrink0-knn200-20.0
 % first => userknn-user-usersim-pcc-shrink10-knn200-20.0
%  \multirow{3}{*}{\algname{UserKNN}} 
%  & $CC_u$         & 16.19\% & 16.11\% & 15.99\% & \bf{16.24\%} & 15.93\% & &  &  &  \\
%  & $LTC_u$        & 15.84\% & 15.75\% & 15.64\% & \bf{15.89\%} & 15.58\% & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   & 16.72\% & 16.28\% & 16.25\% & 16.37\% & 16.33\% & &  &  &  \\
%  & $LTC_{ubest}$  & 16.37\% & 15.93\% & 15.89\% & 16.02\% & 15.97\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.538   & 0.539   & 0.543   & 0.537   & 0.538   & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}

% \multirow{3}{*}{\algname{ItemKNN}} 
%  & $CC_u$         & 6.43\% & 7.04\% & \bf{7.19\%} & 6.96\% & 6.93\% & &  &  &  \\
%  & $LTC_u$        & 6.04\% & 6.65\% & \bf{6.80\%} & 6.57\% & 6.54\% & &  &  &  \\
%  & $CC_i$         &  & 6.81\% & 6.71\% & 6.82\% & 6.68\% & &  &  &  \\
%  & $LTC_i$        &  & 6.42\% & 6.32\% & 6.43\% & 6.29\% & &  &  &  \\
 % rate => itemknn-user-itemsim-cos-shrink0-knn40-20.0
 % zscore,first,ceil,last => itemknn-user-itemsim-cos-shrink0-knn20-20.0
%  & $CC_{ubest}$   & 45.75\% & 52.95\% & 51.68\% & 51.83\% & 51.92\% & &  &  &  \\
%  & $LTC_{ubest}$  & 45.52\% & 52.75 & 51.47\% & 51.63\% & 51.71\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.028 & 0.015 & 0.009 & 0.011 & 0.012 & &  &  &  \\
% zscore,first,ceil,last => itemknn-item-itemsim-cos-shrink0-knn20-20.0
%  & $CC_{ibest}$   &  & 51.49\% & 51.19\% & 50.45\% & 51.28\% & &  &  &  \\
%  & $LTC_{ibest}$  &  & 51.29\% & 50.98\% & 50.87\% & 51.07\% & &  &  &  \\
%  & $nDCG_{ibest}$ &  & 0.015 & 0.011 & 0.011 & 0.012 & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{SLIM}} 
%  & $CC_u$         & 6.27\% & 38.60\% & 1.25\% & 1.34\% & 1.45\% & &  &  &  \\
%  & $LTC_u$        & 6.27\% & 38.60\% & 1.34\% & 1.34\% & 1.45\% & &  &  &  \\
%  & $CC_i$         &  & 35.73\% & 1.25\% & 1.25\% & 1.25\% & &  &  &  \\
%  & $LTC_i$        &  & 35.46\% & 0.93\% & 0.93\% & 0.93\% & &  &  &  \\
% rate => slim-item-itemsim-cos-knn50-itemax100-l10.05-l22-20.0
% zscore => slim-user-itemsim-cos-knn50-itemax100-l10.5-l25-20.0
% first,ceil,last => slim-user-itemsim-cos-knn100-itemax30-l10.05-l25-20.0
%  & $CC_{ubest}$   & 57.48\% & 54.93\% & 46.89\% & 52.45\% & 54.16\% & &  &  &  \\
%  & $LTC_{ubest}$  & 57.32\% & 54.74\% & 46.68\% & 52.26\% & 53.96\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.077 & 0.160 & 0.273 & 0.267 & 0.264 & &  &  &  \\
% zscore => slim-item-itemsim-cos-knn50-itemax100-l10.05-l25-20.0
% first,ceil,last => slim-item-itemsim-cos-knn100-itemax30-l10.05-l25-20.0
%  & $CC_{ibest}$   &  & 55.44\% & 54.57\% & 57.04\% & 52.97\% & &  &  &  \\
%  & $LTC_{ibest}$  &  & 55.26\% & 54.38\% & 56.86\% & 52.77\% & &  &  &  \\
%  & $nDCG_{ibest}$ &  & 0.024 & 0.280 & 0.271 & 0.268 & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{BiasedMF}} 
%  & $CC_u$         & 13.21\% & 11.44\% & 1.87\% & 1.84\% & 6.61\% & &  &  &  \\
%  & $LTC_u$        & 12.79\% & 11.04\% & 1.57\% & 1.54\% & 6.21\% & &  &  &  \\
%  & $CC_i$         &  & 30.80\% & 17.34\% & 15.26\% & 15.18\% & &  &  &  \\
%  & $LTC_i$        &  & 29.20\% & 16.99\% & 14.91\% & 14.55\% & &  &  &  \\
% rate => biasedmf-user-u0.01-i0.01-bias0.01-itemax30-itelearn0.0001-fac150-20.0
% zscore => biasedmf-user-u0.001-i0.001-bias0.001-itemax30-itelearn0.0001-fac150-20.0
% first,ceil,last => biasedmf-user-u0.01-i0.01-bias0.01-itemax100-itelearn0.005-fac100-20.0
%  & $CC_{ubest}$   & 52.30\% & 52.11\% & 30.30\% & 33.22\% & 34.71\% & &  &  &  \\
%  & $LTC_{ubest}$  & 47.98\% & 47.80\% & 28.87\% & 32.06\% & 34.47\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.013 & 0.021 & 0.066 & 0.060 & 0.046 & &  &  &  \\
% zscore => biasedmf-item-u0.01-i0.01-bias0.01-itemax100-itelearn0.001-fac150-20.0
% first,ceil => biasedmf-item-u0.001-i0.001-bias0.001-itemax30-itelearn0.0001-fac150-20.0
% last => biasedmf-item-u0.01-i0.01-bias0.01-itemax100-itelearn0.005-fac100-20.0
% smoothed => biasedmf-item-u0.005-i0.005-bias0.005-itemax100-itelearn0.005-fac100-20.0
  & $CC_{ibest}$   & 52.30\% & 61.71\% & 40.80\% & 43.49\% & 21.86\% & & 34.20\% & 32.27\% & 31.15\% \\
%  & $LTC_{ibest}$  &  & 57.16\% & 38.21\% & 40.41\% & 21.54\% & & 33.93\% & 31.98\% & 30.86\% \\
  & $nDCG_{ibest}$ & 0.013 & 0.062 & 0.143 & 0.179 & 0.040 & & 0.028 & 0.033 & 0.040 \\

 \cline{1-11}
 
% \multirow{3}{*}{\algname{ListRank}} 
%  & $CC_u$         & 4.69\% & 8.56\% & 7.90\% & 7.41\% & 7.69\% & &  &  &  \\
%  & $LTC_u$        & 4.25\% & 7.87\% & 7.49\% & 7.02\% & 7.29\% & &  &  &  \\
%  & $CC_i$         &  & 7.54\% & 6.88\% & 4.61\% & 11.35\% & &  &  &  \\
%  & $LTC_i$        &  & 6.94\% & 6.27\% & 4.16\% & 10.85\% & &  &  &  \\
% rate => listrankmf-user-u0.005-i0.005-itemax100-itelearn0.005-fac150-20.0
% zscore => listrankmf-user-u0.005-i0.005-itemax30-itelearn0.005-fac150-20.0
% first,ceil => listrankmf-user-u0.005-i0.005-itemax100-itelearn0.001-fac100-20.0
% last => listrankmf-user-u0.005-i0.005-itemax100-itelearn0.005-fac150-20.0
%  & $CC_{ubest}$   & 18.45\% & 17.40\% & 20.22\% & 21.10\% & 21.79\% & &  &  &  \\
%  & $LTC_{ubest}$  & 18.11\% & 16.52\% & 19.89\% & 20.77\% & 21.46\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.205 & 0.234 & 0.173 & 0.188 & 0.184 & &  &  &  \\
% zscore => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.001-fac50-20.0
% first => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.0001-fac100-20.0
% ceil => listrankmf-item-u0.001-i0.001-itemax100-itelearn0.0001-fac50-20.0     
% last => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.0001-fac50-20.0     
%  & $CC_{ibest}$   &  & 17.46\% & 17.82\% & 20.39\% & 17.06\% & &  &  &  \\
%  & $LTC_{ibest}$  &  & 16.11\% & 16.59\% & 18.78\% & 15.65\% & &  &  &  \\
%  & $nDCG_{ibest}$ &  & 0.042 & 0.008 & 0.170 & 0.031 & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{SVD++}} 
%  & $CC_u$         & 36.08\% & 29.56\% & 18.33\% & 16.71\% & 22.09\% & & 16.78\% & 17.18\% & 17.55\% \\
%  & $LTC_u$        & 33.92\% & 27.82\% & 17.99\% & 16.36\% & 21.76\% & & 16.43\% & 16.84\% & 17.20\% \\
%  & $CC_i$         &  & 35.62\% & 21.19\% & 19.65\% & 16.51\% & &  &  &  \\
%  & $LTC_i$        &  & 33.18\% & 20.67\% & 19.13\% & 15.40\% & &  &  &  \\
% rate => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.0001-fac150-20.0
% zscore => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.0001-fac150-20.0
% first => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
% ceil => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.001-fac50-20.0
% last => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
%  & $CC_{ubest}$   & 61.30\% & 60.36\% & 18.33\% & 18.18\% & 22.09\% & &  &  &  \\
%  & $LTC_{ubest}$  & 56.43\% & 55.57\% & 17.99\% & 17.84\% & 21.76\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.007 & 0.013 & 0.079 & 0.080 & 0.124 & &  &  &  \\
% rate => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.001-fac150-20.0
% first => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% ceil => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% last => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% smoothed first,ceil => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.001-fac150-20.0
% smoothed last => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
  & $CC_{ibest}$   & 61.30\% & 67.13\% & 33.32\% & 37.08\% & 18.71\% & & 24.11\% & 23.07\% & 21.22\% \\
%  & $LTC_{ibest}$  &  & 62.14\% & 31.85\% & 34.99\% & 17.57\% & & 23.80\% & 22.74\% & 20.89\% \\
  & $nDCG_{ibest}$ & 0.007 & 0.015 & 0.164 & 0.202 & 0.223 & & 0.028 & 0.041 & 0.039 \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{NMF}}
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/coverage_table5.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms in terms of item coverage on ML1M dataset } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{metrics} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & zscore & first & ceil & last & & first & ceil & last \\
 \bottomrule
%  \multirow{3}{*}{\algname{UserKNN}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{ItemKNN}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{SLIM}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{BiasedMF}} 
%  & $CC_u$         & 2.67\% & 2.87\% & 9.75\% & 10.02\% & 13.21\% & &  &  &  \\
%  & $LTC_u$        & 1.51\% & 1.68\% & 7.20\% & 7.38\% & 10.53\% & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% rate,zscore => biasedmf-user-u0.01-i0.01-bias0.01-itemax100-itelearn0.01-fac50-20.0  
% first,last => biasedmf-user-u0.01-i0.01-bias0.01-itemax30-itelearn0.001-fac50-20.0
% ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.001-fac50-20.0
%  & $CC_{ubest}$   & 64.76\% & 63.08\% & 56.25\% & 65.11\% & 71.75\% & &  &  &  \\
%  & $LTC_{ubest}$  & 63.72\% & 61.98\% & 55.03\% & 64.04\% & 70.92\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.033 & 0.032 & 0.039 & 0.030 & 0.021 & &  &  &  \\
% zscore => biasedmf-item-u0.01-i0.01-bias0.01-itemax30-itelearn0.001-fac150-20.0
% first,ceil => biasedmf-item-u0.001-i0.001-bias0.001-itemax100-itelearn0.005-fac50-20.0
% last => biasedmf-item-u0.01-i0.01-bias0.01-itemax30-itelearn0.001-fac50-20.0
% smoothed first => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% smoothed ceil => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.005-fac50-20.0
% smoothed last => biasedmf-item-u0.005-i0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
  & $CC_{ibest}$   & 64.76\% & 89.47\% & 80.32\% & 86.96\% & 70.65\% & & 81.63\% & 85.48\% & 68.94\% \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ & 0.033 & 0.010 & 0.006 & 0.010 & 0.024 & & 0.008 & 0.011 & 0.031 \\
  
 \cline{1-11}
 
% \multirow{3}{*}{\algname{ListRank}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{SVD++}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{NMF}}
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/coverage_table6.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms in terms of item coverage on Yelp dataset } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{metrics} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & zscore & first & ceil & last & & first & ceil & last \\
 \bottomrule
%  \multirow{3}{*}{\algname{UserKNN}} 
%  & $CC_u$         & 52.48\% & 53.47\% & 52.99\% & 52.94\% & 53.11\% & &  &  &  \\
%  & $LTC_u$        & 51.23\% & 52.24\% & 51.74\% & 51.70\% & 51.87\% & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% rate => userknn-user-usersim-pcc-shrink20-knn50-20.0
% zscore,first,ceil,last => userknn-user-usersim-pcc-shrink10-knn70-20.0
%  & $CC_{ubest}$   & 53.47\% & 54.94\% & 54.75\% & 54.52\% & 54.75\% & &  &  &  \\
%  & $LTC_{ubest}$  & 52.24\% & 53.75\% & 53.56\% & 53.32\% & 53.55\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.024 & 0.024 & 0.024 & 0.023 & 0.023 & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{ItemKNN}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         & 12.33\% & 12.46\% & 14.53\% & 13.52\% & 13.13\% & &  &  &  \\
%  & $LTC_i$        & 10.03\% & 10.16\% & 12.28\% & 11.25\% & 10.85\% & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
% all => itemknn-item-itemsim-cos-shrink0-knn10-20.0
%  & $CC_{ibest}$   & 66.46\% & 69.32\% & 68.62\% & 68.48\% & 68.29\% & &  &  &  \\
%  & $LTC_{ibest}$  & 65.58\% & 68.51\% & 67.79\% & 67.64\% & 67.45\% & &  &  &  \\
%  & $nDCG_{ibest}$ & 0.007 & 0.007 & 0.006 & 0.006 & 0.006 & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{SLIM}} 
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{BiasedMF}} 
  & $CC_u$         &  &  &  &  &  & &  &  &  \\
  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
  & $CC_i$         &  &  &  &  &  & &  &  &  \\
  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
 \cline{1-11}
 
% \multirow{3}{*}{\algname{ListRank}} 
%  & $CC_u$         & 18.66\% & 0.45\% & 26.24\% & 23.52\% & 21.07\% & &  &  &  \\
%  & $LTC_u$        & 16.54\% & 0.03\% & 24.31\% & 21.54\% & 19.05\% & &  &  &  \\
%  & $CC_i$         &  &  &  &  & & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
% rate,zscore => listrankmf-user-u0.01-i0.01-itemax100-itelearn0.001-fac150-20.0
% first,ceil,last => listrankmf-user-u0.001-i0.001-itemax100-itelearn0.0001-fac150-20.0
%  & $CC_{ubest}$   & 39.51\% & 24.86\% & 43.41\% & 38.72\% & 35.75\%  & &  &  &  \\
%  & $LTC_{ubest}$  & 37.91\% & 22.87\% & 41.91\% & 37.10\% & 34.05\% & &  &  &  \\
%  & $nDCG_{ubest}$ & 0.013 & 0.014 & 0.013 & 0.013 & 0.014 & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
 \multirow{3}{*}{\algname{SVD++}} 
  & $CC_u$         &  &  &  &  &  & &  &  &  \\
  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
  & $CC_i$         &  &  &  &  &  & &  &  &  \\
  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
% \cline{1-11}
 
% \multirow{3}{*}{\algname{NMF}}
%  & $CC_u$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_u$        &  &  &  &  &  & &  &  &  \\
%  & $CC_i$         &  &  &  &  &  & &  &  &  \\
%  & $LTC_i$        &  &  &  &  &  & &  &  &  \\
%  & $CC_{ubest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ubest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ubest}$ &  &  &  &  &  & &  &  &  \\
%  & $CC_{ibest}$   &  &  &  &  &  & &  &  &  \\
%  & $LTC_{ibest}$  &  &  &  &  &  & &  &  &  \\
%  & $nDCG_{ibest}$ &  &  &  &  &  & &  &  &  \\
  
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/ndcg_table1.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms at nDCG@10 } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule
 \multirow{2}{*}{dataset} & \multirow{2}{*}{algorithms} &  &  & \multicolumn{3}{c}{\bf{Percentile}} & & \multicolumn{3}{c}{\bf{Smoothed Percentile ($k=5$)}} \\\cline{5-7}\cline{9-11}
  
 
 & & rate & $zscore_u$ & $first_u$ & $ceil_u$ & $last_u$ & & $first_u$ & $ceil_u$ & $last_u$ \\
 \bottomrule
 
 % all => userknn-user-usersim-pcc-shrink20-knn10-20.0   
 \multirow{14}{*}{BX} & \algname{UserKNN} & 0.015 & 0.016 & 0.016 & 0.016 & 0.016 & & 0.016 & 0.016 & 0.016 \\
 % first,floor,ceil,last,zscore => userknn-item-usersim-pcc-shrink20-knn10-20.0
  &  &  & 0.032 & 0.032 & 0.032 & 0.031 & &  &  &  \\
  

% rate => itemknn-item-itemsim-cos-shrink20-knn10-20.0
% all => itemknn-user-itemsim-cos-shrink20-knn10-20.0
 & \algname{ItemKNN} & 0.059 & 0.059 & 0.061 & 0.061 & 0.061 & &  &  &  \\
% all => itemknn-item-itemsim-cos-shrink20-knn10-20.0
 &  &  & 0.059 & \bf{0.061} & \bf{0.061} & \bf{0.061} & & 0.061 & 0.061 & 0.061 \\


% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% first,ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
% last => biasedmf-user-u0.005-i0.005-bias0.005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac100-20.0
 & \algname{BiasedMF} & 0.009 & 0.008 & \bf{0.014} & \bf{0.014} & \bf{0.012} & & \bf{0.014} & \bf{0.014} & \bf{0.013} \\
% zscore => biasedmf-item-u0.005-i0.005-bias0.005-itemax50-itelearn0.005-fac50-20.0
% first,ceil,last => biasedmf-item-u0.005-i0.005-bias0.005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => biasedmf-item-u0.005-i0.005-bias0.005-itemax30-itelearn0.001-fac150-20.0
 &  &  & 0.004 & \bf{0.009} & \bf{0.012} & \bf{0.013} & & 0.007 & 0.008 & 0.010 \\  
  

% rate => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.01-fac150-20.0
% zscore => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.001-fac100-20.0
% first => listrankmf-user-u0.01-i0.01-itemax100-itelearn0.001-fac150-20.0
% ceil,last => listrankmf-user-u0.01-i0.01-itemax100-itelearn0.001-fac150-20.0
% smoothed all => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.0001-fac150-20.0
 & \algname{ListRank} & 0.013 & 0.014 & 0.012 & 0.012 & 0.013 & & 0.009 & 0.010 & 0.011 \\
% zscore => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.005-fac100-20.0
% first => listrankmf-item-u0.0001-i0.0001-itemax30-itelearn0.01-fac150-20.0
% ceil => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.001-fac100-20.0
% last => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.0001-fac50-20.0
 &  &  & 0.013 & 0.013 & 0.013 & 0.010 & &  &  &  \\


% rate => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
% first,ceil,last => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.0001-fac50-20.0
% smoothe all => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0                
 & \algname{SVD++} & 0.009 & 0.006 & \bf{0.011} & \bf{0.011} & \bf{0.010} & & \bf{0.014} & \bf{0.013} & \bf{0.012} \\
% zscore => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax50-itelearn0.005-fac50-20.0
% first => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.0001-fac150-20.0
%ceil,last => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax50-itelearn0.0001-fac150-20.0
% smoothed all => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.0001-fac150-20.0
 &  &  & 0.005 & \bf{0.017} & \bf{0.014} & \bf{0.016} & & 0.007 & 0.009 & 0.011 \\


%rate => nmf-user--itemax100-fac100-20.0
% zscore => nmf-user--itemax100-fac50-20.0
% first => nmf-user--itemax50-fac50-20.0
% ceil => nmf-user--itemax100-fac100-20.0
% last => nmf-user--itemax100-fac100-20.0
% smoothed first,ceil => nmf-user--itemax100-fac50-20.0
% smoothed last => nmf-user--itemax100-fac100-20.0
 & \algname{\color{red}NMF} & 0.0005 & 0.0004 & 0.0005 & \bf{0.0006} & \bf{0.0007} & & 0.0005 & \bf{0.0006} & \bf{0.0006} \\
% first => nmf-item--itemax100-fac100-20.0
% ceil,last => nmf-item--itemax100-fac150-20.0
% zscore => nmf-item--itemax30-fac150-20.0
% smoothed all => nmf-item--itemax100-fac100-20.0
 &  &  & 0.0005 & \bf{0.0006} & \bf{0.0006} & \bf{0.0006} & & \bf{0.0006} & \bf{0.0006} & \bf{0.0006} \\


 & \algname{SLIM} &  &  &  &  &  & &  &  &  \\

 &  &  &  &  &  &  & &  &  &  \\

\cline{1-11}


% rate,zscore,first,last => userknn-user-usersim-pcc-shrink10-knn10-20.0
% ceil => userknn-user-usersim-pcc-shrink20-knn10-20.0
% smoothed => userknn-user-usersim-pcc-shrink10-knn10-20.0  
  \multirow{7}{*}{CiaoDVD} & \algname{UserKNN} & 0.0097 & 0.0099 & 0.0097 & 0.0098 & 0.0097 & & 0.010 & 0.010 & 0.010 \\
% rate,zscore,last => userknn-item-usersim-pcc-shrink20-knn10-20.0
% first,ceil => userknn-item-usersim-pcc-shrink10-knn10-20.0
% smoothed => userknn-item-usersim-pcc-shrink20-knn10-20.0 
  &  & & 0.0117 & \bf{0.0125} &0.0117 & \bf{0.0124} & & \bf{0.013} & \bf{0.012} & \bf{0.013} \\
  
  
% all => itemknn-user-itemsim-cos-shrink20-knn10-20.0
% smoothed => itemknn-user-itemsim-cos-shrink20-knn30-20.0
 & \algname{ItemKNN} & 0.034 & 0.034 & 0.033 & 0.034 & 0.033 & & 0.034 & 0.034 & 0.034 \\
% all => itemknn-item-itemsim-cos-shrink20-knn40-20.0     
% smoothed => itemknn-item-itemsim-cos-shrink20-knn30-20.0
  &  &  & 0.034 &0.033 & 0.033 & 0.034 & & 0.033 & 0.034 & 0.034 \\


% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.001-fac50-20.0
% first,last => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac50-20.0
% ceil => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac100-20.0
% smoothed all => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
 & \algname{BiasedMF} & 0.019 & 0.005 & \bf{0.027} & \bf{0.024} & 0.016 & & \bf{0.027} & \bf{0.027} & \bf{0.026} \\
 &  &  &  &  &  &  & &  &  &  \\
 
 
% rate => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.01-fac150-20.0
% zscore => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.005-fac150-20.0
% first => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.005-fac100-20.0
% ceil => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.005-fac100-20.0
% last => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.005-fac100-20.0
% smoothed first => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.005-fac150-20.0
% smoothed ceil => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.005-fac150-20.0
% smoothed last => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.01-fac150-20.0
 & \algname{ListRank} & 0.019 & 0.019 & \bf{0.022} & \bf{0.022} & \bf{0.023} & & \bf{0.025} & \bf{0.025} & \bf{0.025} \\
% zscore => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.005-fac150-20.0
% first => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.01-fac150-20.0
% ceil => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.001-fac100-20.0
% last => listrankmf-item-u0.0001-i0.0001-itemax30-itelearn0.0001-fac100-20.0
&  &  & 0.027 & 0.022 & 0.023 & 0.021 & &  &  &  \\


% rate => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.001-fac50-20.0
% zscore => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax50-itelearn0.005-fac100-20.0
% first,ceil => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.0001-fac50-20.0
% last => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
 & \algname{SVD++} & 0.009 & 0.011 & \bf{0.022} & \bf{0.019} & \bf{0.017} & & \bf{0.019} & \bf{0.018} & \bf{0.016} \\
 &  &  &  &  &  &  & &  &  &  \\


% rate => nmf-item--itemax100-fac100-20.0   
% zscore => nmf-user--itemax30-fac100-20.0
% first,ceil,last => nmf-user--itemax100-fac50-20.0
 & \algname{\color{red}NMF} & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & &  &  &  \\
% zsccore => nmf-item--itemax100-fac100-20.0   
% first,ceil,last => nmf-item--itemax30-fac50-20.0
% smoothed => nmf-item--itemax50-fac100-20.0
 &  &  & 0.0001 & 0.0001 & 0.0001 & 0.0001 & & 0.0001 & 0.0001 & 0.0001 \\


% rate => slim-item-itemsim-cos-knn100-itemax100-l10.05-l25-20.0
% zscore => slim-user-itemsim-cos-knn100-itemax50-l10.05-l22-20.0
% first => slim-user-itemsim-cos-knn50-itemax30-l10.05-l25-20.0
% ceil => slim-user-itemsim-cos-knn50-itemax30-l15-l25-20.0
% last => slim-user-itemsim-cos-knn100-itemax30-l10.5-l25-20.0
% smoothed first -> slim-user-itemsim-cos-knn50-itemax30-l15-l25-20.0
% smoothed ceil -> slim-user-itemsim-cos-knn50-itemax30-l12-l25-20.0
% smoothed last -> slim-user-itemsim-cos-knn100-itemax30-l12-l25-20.0
 & \algname{\color{red}SLIM} & 0.005 & 0.005 & 0.003 & 0.003 & 0.002 & & 0.004 & 0.003 & 0.003 \\
% zscore => slim-item-itemsim-cos-knn100-itemax100-l10.05-l25-20.0
% first,ceil,last => slim-item-itemsim-cos-knn50-itemax30-l10.5-l25-20.0
% smoothed all => slim-item-itemsim-cos-knn50-itemax30-l12-l25-20.0
 &  &  & 0.006 & 0.003 & 0.003 & 0.004 & & 0.003  & 0.003 & 0.003 \\ 
 
 
 \cline{1-11}


% all => userknn-user-usersim-pcc-shrink20-knn20-20.0   
 \multirow{7}{*}{Epinions} & \algname{UserKNN} & 0.068 & 0.068 & 0.068 & 0.068 & 0.068 & & 0.068 & 0.068 & 0.068 \\
% all => userknn-item-usersim-pcc-shrink20-knn20-20.0
  &  &  & 0.067 & 0.069 & 0.067 & 0.068 & &  &  &  \\

% rate => itemknn-item-itemsim-cos-shrink20-knn100-20.0
% zscore,first,ceil.last => itemknn-user-itemsim-cos-shrink20-knn40-20.0
 & \algname{ItemKNN} & 0.071 & 0.070 & 0.070 & 0.070 & 0.070 & &  &  &  \\
% all => itemknn-item-itemsim-cos-shrink20-knn20-20.0
% smoothed first => itemknn-item-itemsim-cos-shrink20-knn50-20.0
% smoothed ceil,last => itemknn-item-itemsim-cos-shrink10-knn10-20.0
 &  &  & 0.070 & 0.070 & 0.071 & 0.070 & & 0.071 & 0.072 & 0.071 \\
 
 
% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac50-20.0
% first => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% smoothed first,last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
% smoothed ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
 & \algname{BiasedMF} & 0.019 & 0.017 & \bf{0.022} & \bf{0.022} & \bf{0.021} & & \bf{0.022} & \bf{0.023} & \bf{0.022} \\
% zscore => biasedmf-item-u0.001-i0.001-bias0.001-itemax30-itelearn0.005-fac50-20.0
% first => biasedmf-item-u0.001-i0.001-bias0.001-itemax30-itelearn0.0001-fac50-20.0
% ceil => biasedmf-item-u0.001-i0.001-bias0.001-itemax50-itelearn0.0001-fac100-20.0
% last => biasedmf-item-u0.001-i0.001-bias0.001-itemax50-itelearn0.0001-fac150-20.0
% smoothed all => biasedmf-item-u0.005-i0.005-bias0.005-itemax100-itelearn0.0001-fac50-20.0
 &  &  & 0.014 & \bf{0.033} & \bf{0.021} & \bf{0.016} & & 0.014 & 0.014 & 0.016 \\
  

% rate,zscore,first,ceil => listrankmf-user-u0.005-i0.005-itemax30-itelearn0.0001-fac100-20.0
% last => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.001-fac150-20.0
% smoothed first => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.01-fac150-20.0
% smoothed ceil => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
% smoothed last => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.001-fac150-20.0
 & \algname{ListRank} & 0.033 & 0.037 & 0.035 & 0.034 & 0.031 & & 0.031 & 0.032 & 0.033 \\
 &  &  &  &  &  &  & &  &  &  \\


 & \algname{SVD++} &  &  &  &  &  & &  &  &  \\
 &  &  &  &  &  &  & &  &  &  \\


% rate,zscore => nmf-user--itemax100-fac100-20.0
% first,ceil,last => nmf-user--itemax100-fac150-20.0
% smoothed first,ceil,last => nmf-user--itemax100-fac100-20.0
 & \algname{\color{red}NMF} & 0.0019 & 0.0015 & 0.0017 & 0.0018 & 0.0020 & & 0.0017 & 0.0017 & 0.0018 \\
 &  &  &  &  &  &  & &  &  &  \\
  

% rate,zscore,first,ceil => slim-user-itemsim-cos-knn100-itemax30-l10.05-l25-20.0
% last => slim-user-itemsim-cos-knn100-itemax50-l15-l20.05-20.0
% smoothed => slim-user-itemsim-cos-knn100-itemax30-l12-l25-20.0
 & \algname{SLIM} & 0.010 & 0.009 & 0.007 & 0.008 & 0.009 & & 0.008 & 0.009 & 0.008 \\
 &  &  &  &  &  &  & &  &  &  \\
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/ndcg_table1_draft.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Performance of recommendation algorithms at nDCG@10 } \label{tab:res1}
\begin{tabular}{llrrrrrrrrrrr}
\toprule
 \multirow{2}{*}{dataset} & \multirow{2}{*}{algorithms} &  &  & \multicolumn{4}{c}{\bf{Percentile}} & & \multicolumn{4}{c}{\bf{Smoothed Percentile ($k=5$)}} \\\cline{5-8}\cline{10-13}
  
 
 & & rate & $zscore_u$ & $first_u$ & $floor_u$ & $ceil_u$ & $last_u$ & & $first_u$ & $floor_u$ & $ceil_u$ & $last_u$ \\
 \bottomrule
 
 %\multirow{8}{*}{BX} & \algname{ItemAVG} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
 % all => userknn-user-usersim-pcc-shrink20-knn10-20.0   
 \multirow{14}{*}{BX} & \algname{UserKNN} & 0.015 & 0.016 & 0.016 & 0.016 & 0.016 & 0.016 & & 0.016 & 0.016 & 0.016 & 0.016 \\
 
 % first,floor,ceil,last,zscore => userknn-item-usersim-pcc-shrink20-knn10-20.0
 % floor => 
 &  &  & 0.032 & 0.032 & 0.033 & 0.032 & 0.031 & &  &  &  &  \\
  
 %\cline{1-14}
 
 & \algname{ItemKNN} &  &  &  &  &  &  & &  &  &  &  \\

 &  &  &  &  &  &  &  & &  &  &  &  \\
%\cline{1-14}
% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% first,floor,ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
% last => biasedmf-user-u0.005-i0.005-bias0.005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac100-20.0
 & \algname{BiasedMF} & 0.009 & 0.008 & \bf{0.014} & \bf{0.014} & \bf{0.014} & \bf{0.012} & & \bf{0.014} & \bf{0.014} & \bf{0.014} & \bf{0.013} \\
% zscore => biasedmf-item-u0.005-i0.005-bias0.005-itemax50-itelearn0.005-fac50-20.0
% first,ceil,last => biasedmf-item-u0.005-i0.005-bias0.005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => biasedmf-item-u0.005-i0.005-bias0.005-itemax30-itelearn0.001-fac150-20.0
 &  &  & 0.004 & \bf{0.009} &  & \bf{0.012} & \bf{0.013} & & 0.007 & 0.008 & 0.008 & 0.010 \\  
  
%\cline{1-14}
% rate => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.0001-fac150-20.0
% zscore => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.001-fac150-20.0
% first => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.0001-fac150-20.0
% floor => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.01-fac150-20.0
% ceil,last => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.001-fac100-20.0
% smoothed all => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.0001-fac150-20.0
 & \algname{ListRank} & 0.011 & 0.011 & 0.009 & 0.010 & 0.009 & 0.009 & & 0.009 & 0.010 & 0.010 & 0.011 \\

% zscore => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.005-fac100-20.0
% first => listrankmf-item-u0.0001-i0.0001-itemax30-itelearn0.01-fac150-20.0
% floor,ceil => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.001-fac100-20.0
% last => listrankmf-item-u0.0001-i0.0001-itemax100-itelearn0.0001-fac50-20.0
 &  &  & 0.013 & 0.013 & 0.013 & 0.013 & 0.010 & &  &  &  &  \\

%\cline{1-14}
% rate => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
% first,floor,ceil,last => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.0001-fac50-20.0
% smoothe all => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0                
 & \algname{SVD++} & 0.009 & 0.006 & \bf{0.011} & \bf{0.011} & \bf{0.011} & \bf{0.010} & & \bf{0.014} & \bf{0.013} & \bf{0.013} & \bf{0.012} \\

% zscore => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax50-itelearn0.005-fac50-20.0
% first => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.0001-fac150-20.0
%ceil,last => svdpp-item--u0.005-i0.005-impItem0.005-bias0.005-itemax50-itelearn0.0001-fac150-20.0
% smoothed all => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.0001-fac150-20.0
 &  &  & 0.005 & \bf{0.017} &  & \bf{0.014} & \bf{0.016} & & 0.007 &  & 0.009 & 0.011 \\

%\cline{1-14}
%rate => nmf-user--itemax100-fac100-20.0
% zscore => nmf-user--itemax100-fac50-20.0
% first => nmf-user--itemax50-fac50-20.0
% floor => nmf-user--itemax50-fac100-20.0
% ceil => nmf-user--itemax100-fac100-20.0
% last => nmf-user--itemax100-fac100-20.0
% smoothed first,floor,ceil => nmf-user--itemax100-fac50-20.0
% smoothed last => nmf-user--itemax100-fac100-20.0
 & \algname{\color{red}NMF} & 0.0005 & 0.0004 & 0.0005 & \bf{0.0006} & \bf{0.0006} & \bf{0.0007} & & 0.0005 & \bf{0.0006} & \bf{0.0006} & \bf{0.0006} \\

% first,floor => nmf-item--itemax100-fac100-20.0
% ceil,last => nmf-item--itemax100-fac150-20.0
% zscore => nmf-item--itemax30-fac150-20.0
% smoothed all => nmf-item--itemax100-fac100-20.0
 &  &  & 0.0005 & \bf{0.0006} & \bf{0.0006} & \bf{0.0006} & \bf{0.0006} & & \bf{0.0006} & 0.0005 & \bf{0.0006} & \bf{0.0006} \\

%\cline{1-14}
 & \algname{SLIM} &  &  &  &  &  &  & &  &  &  &  \\

 &  &  &  &  &  &  &  & &  &  &  &  \\

\cline{1-13}

%\multirow{8}{*}{CiaoDVD} & \algname{ItemAVG} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
 % rate,zscore,first,last => userknn-user-usersim-pcc-shrink10-knn10-20.0
  % floor,ceil => userknn-user-usersim-pcc-shrink20-knn10-20.0
  \multirow{7}{*}{CiaoDVD} & \algname{UserKNN} & 0.0097 & 0.0099 & 0.0097 & 0.0098 & 0.0098 & 0.0097 & &  &  &  &  \\
  
% rate,zscore,last => userknn-item-usersim-pcc-shrink20-knn10-20.0
 % first,floor,ceil => userknn-item-usersim-pcc-shrink10-knn10-20.0
  &  & & 0.0117 & \bf{0.0125} & 0.0119 & 0.0117 & \bf{0.0124} & &  &  &  &  \\
  
 %\cline{1-14}
 
 & \algname{ItemKNN} &  &  &  &  &  &  & &  &  &  &  \\
 
 % all => itemknn-item-itemsim-cos-shrink20-knn40-20.0              
  &  & 0.034 & 0.034 & 0.033 & 0.033 & 0.033 & 0.034 & &  &  &  &  \\

%\cline{1-14}
% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.001-fac50-20.0
% first,last => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac50-20.0
% floor,ceil => biasedmf-user-u0.005-i0.005-bias0.005-itemax30-itelearn0.0001-fac100-20.0
% smoothed all => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
 & \algname{BiasedMF} & 0.019 & 0.005 & \bf{0.027} & \bf{0.023} & \bf{0.024} & 0.016 & & \bf{0.027} & \bf{0.026} & \bf{0.027} & \bf{0.026} \\
  
%\cline{1-14}
% rate => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.01-fac150-20.0
% zscore => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.005-fac150-20.0
% first => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.005-fac100-20.0
% floor => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.0001-fac100-20.0
% ceil => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.005-fac100-20.0
% last => listrankmf-user-u0.0001-i0.0001-itemax30-itelearn0.005-fac100-20.0
% smoothed first => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.005-fac150-20.0
% smoothed floor => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
% smoothed ceil => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.005-fac150-20.0
% smoothed last => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.01-fac150-20.0
 & \algname{ListRank} & 0.019 & 0.019 & \bf{0.022} & \bf{0.023} & \bf{0.022} & \bf{0.023} & & \bf{0.025} & \bf{0.024} & \bf{0.025} & \bf{0.025} \\

% zscore => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.005-fac150-20.0
% first => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.01-fac150-20.0
% ceil => listrankmf-item-u0.0001-i0.0001-itemax50-itelearn0.001-fac100-20.0
% last => listrankmf-item-u0.0001-i0.0001-itemax30-itelearn0.0001-fac100-20.0
&  &  & 0.027 & 0.022 &  & 0.023 & 0.021 & &  &  &  &  \\

%\cline{1-14}
% rate => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.001-fac50-20.0
% zscore => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax50-itelearn0.005-fac100-20.0
% first,floor,ceil => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax30-itelearn0.0001-fac50-20.0
% last => svdpp-user--u0.0005-i0.0005-impItem0.0005-bias0.0005-itemax100-itelearn0.0001-fac150-20.0
% smoothed all => svdpp-user--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
 & \algname{SVD++} & 0.009 & 0.011 & \bf{0.022} & \bf{0.016} & \bf{0.019} & \bf{0.017} & & \bf{0.019} & \bf{0.018} & \bf{0.018} & \bf{0.016} \\

%\cline{1-14}

 & \algname{NMF} &  &  &  &  &  &  & &  &  &  &  \\
  
%\cline{1-14}
% rate => slim-item-itemsim-cos-knn100-itemax100-l10.05-l25-20.0
% zscore => slim-user-itemsim-cos-knn100-itemax50-l10.05-l22-20.0
% first => slim-user-itemsim-cos-knn50-itemax30-l10.05-l25-20.0
% ceil => slim-user-itemsim-cos-knn50-itemax30-l15-l25-20.0
% last => slim-user-itemsim-cos-knn100-itemax30-l10.5-l25-20.0
% smoothed first -> slim-user-itemsim-cos-knn50-itemax30-l15-l25-20.0
% smoothed floor -> slim-user-itemsim-cos-knn100-itemax30-l15-l22-20.0
% smoothed ceil -> slim-user-itemsim-cos-knn50-itemax30-l12-l25-20.0
% smoothed last -> slim-user-itemsim-cos-knn100-itemax30-l12-l25-20.0
 & \algname{\color{red}SLIM} & 0.005 & 0.005 & 0.003 &  & 0.003 & 0.002 & & 0.004 & 0.003 & 0.003 & 0.003 \\
 
% zscore =>
% zscore => slim-item-itemsim-cos-knn100-itemax100-l10.05-l25-20.0
% first,floor,ceil,last => slim-item-itemsim-cos-knn50-itemax30-l10.5-l25-20.0
% smoothed all => slim-item-itemsim-cos-knn50-itemax30-l12-l25-20.0
 &  &  & 0.006 & 0.003 & 0.004 & 0.003 & 0.004 & & 0.003 & 0.003 & 0.003 & 0.003 \\ 
 
 \cline{1-13}

%\multirow{8}{*}{Epinions} & \algname{ItemAVG} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
% all => userknn-user-usersim-pcc-shrink20-knn20-20.0            
 \multirow{7}{*}{Epinions} & \algname{UserKNN} & 0.068 & 0.068 & 0.068 &  & 0.068 & 0.068 & &  &  &  &  \\
  
 %\cline{1-14}
 
 & \algname{ItemKNN} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}
% rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac50-20.0
% first => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% floor => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
% smoothed first,floor,last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
% smoothed ceil => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac150-20.0
 & \algname{BiasedMF} & 0.019 & 0.017 & \bf{0.022} & \bf{0.022} & \bf{0.022} & \bf{0.021} & & \bf{0.022} & \bf{0.022} & \bf{0.023} & \bf{0.022} \\

% zscore => biasedmf-item-u0.001-i0.001-bias0.001-itemax30-itelearn0.005-fac50-20.0
% first => biasedmf-item-u0.001-i0.001-bias0.001-itemax30-itelearn0.0001-fac50-20.0
% ceil => biasedmf-item-u0.001-i0.001-bias0.001-itemax50-itelearn0.0001-fac100-20.0
% last => biasedmf-item-u0.001-i0.001-bias0.001-itemax50-itelearn0.0001-fac150-20.0
% smoothed all => biasedmf-item-u0.005-i0.005-bias0.005-itemax100-itelearn0.0001-fac50-20.0
 &  &  & 0.014 & \bf{0.033} &  & \bf{0.021} & \bf{0.016} & & 0.014 &  & 0.014 & 0.016 \\
  
%\cline{1-14}
% rate => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
% zscore => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.001-fac100-20.0
% first => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.001-fac150-20.0
% ceil => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.005-fac150-20.0
% last => listrankmf-user-u0.0001-i0.0001-itemax100-itelearn0.001-fac150-20.0
% smoothed first => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.01-fac150-20.0
% smoothed ceil => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
% smoothed last => listrankmf-user-u0.0001-i0.0001-itemax50-itelearn0.001-fac150-20.0
 & \algname{ListRank} & 0.031 & 0.033 & 0.033 &  & 0.032 & 0.031 & & 0.031 &  & 0.032 & 0.033 \\

%\cline{1-14}

 & \algname{SVD++} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}
% rate,zscore => nmf-user--itemax100-fac100-20.0
% first,floor,ceil,last => nmf-user--itemax100-fac150-20.0
% smoothed first,ceil,last => nmf-user--itemax100-fac100-20.0
% smoothed floor => nmf-user--itemax100-fac150-20.0
 & \algname{\color{red}NMF} & 0.0019 & 0.0015 & 0.0017 & 0.0018 & 0.0018 & 0.0020 & & 0.0017 & 0.0017 & 0.0017 & 0.0018 \\
  
%\cline{1-14}
 & \algname{SLIM} &  &  &  &  &  &  & &  &  &  &  \\
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/ndcg_table2.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
%\captionof{table}{Performance of recommendation algorithms at nDCG@10 } \label{tab:res1}
\begin{tabular}{llrrrrrrrrr}
\toprule


% all -> userknn-user-usersim-pcc-shrink20-knn200-20.0 
 \multirow{9}{*}{FilmTrust} & \algname{\color{red}UserKNN} & 0.543 & 0.544 & 0.543 & 0.542 & 0.542 & & 0.543 & 0.544 & 0.543 \\
 
 
 % rate,zscore,first => itemknn-user-itemsim-cos-shrink20-knn30-20.0
 % ceil => itemknn-user-itemsim-cos-shrink20-knn200-20.0
 % last => itemknn-user-itemsim-cos-shrink20-knn70-20.0
 % smoothed => itemknn-user-itemsim-cos-shrink20-knn40-20.0
 & \algname{\color{red}ItemKNN} & 0.537 & 0.557 & 0.514 & 0.502 & 0.483 & & 0.533 & 0.531 & 0.528 \\
% zscore => itemknn-item-itemsim-cos-shrink20-knn10-20.0
% first,ceil => itemknn-item-itemsim-cos-shrink20-knn50-20.0
% last => itemknn-item-itemsim-cos-shrink20-knn40-20.0
% smoothed first,last => itemknn-item-itemsim-cos-shrink20-knn40-20.0
% smoothed ceil => itemknn-item-itemsim-cos-shrink20-knn70-20.0
&  &  & 0.563 & 0.503 & 0.503 & 0.489 & & 0.496 & 0.497 & 0.485 \\


%rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% first => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
% ceil -> biasedmf-user-u0.001-i0.001-bias0.001-itemax30-itelearn0.0001-fac50-20.0
% last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% smoothed first -> biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0 
% smoothed ceil,last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
 & \algname{BiasedMF} & 0.078 & 0.092 & \bf{0.317} & \bf{0.314} & \bf{0.302} & & \bf{0.352} & \bf{0.345} & \bf{0.335} \\
% first,ceil => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0 
% zscore => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% last, smoothed last => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% smoothed first,ceil => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
 &  &  & 0.167 & \bf{0.215} & \bf{0.234} & \bf{0.270} & & \bf{0.174} & \bf{0.197} & \bf{0.230} \\
 
 

% rate => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac100-20.0
% zscore => listrankmf-user-u0.005-i0.005-itemax30-itelearn0.001-fac50-20.0
% first,ceil,last => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac150-20.0
% smoothed first,last => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac150-20.0
% smoothed ceil => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac100-20.0
 & \algname{\color{red}ListRank} & 0.412 & 0.459 & 0.393 & 0.382 & 0.380 & & 0.394 & 0.397 & 0.412 \\
% zscore => listrankmf-item-u0.001-i0.001-itemax30-itelearn0.01-fac50-20.0
% first => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac50-20.0
% ceil => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac150-20.0
% last => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.001-fac50-20.0
% smoothed first,last => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac50-20.0
% smoothed ceil => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.001-fac50-20.0
 &  &  & 0.448 & 0.445 & 0.457 & 0.397 & & 0.455 & 0.395 & 0.422 \\


% rate => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% zscore => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% first => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
% ceil => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
% last => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
% smoothed => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
 & \algname{SVD++} & 0.049 & 0.072 & \bf{0.079} & \bf{0.087} & \bf{0.124} & & \bf{0.081} & \bf{0.092} & \bf{0.102} \\
% zscore => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.001-fac50-20.0
% first => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% ceil = > svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.0001-fac50-20.0
% last => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0  
% smoothed all => svdpp-item--u0.001-i0.001-impItem0.001-bias0.001-itemax30-itelearn0.0001-fac50-20.0
 &  &  & 0.091 & \bf{0.193} & \bf{0.222} & \bf{0.228} & & \bf{0.080} & \bf{0.107} & \bf{0.143} \\


% rate -> nmf-user--itemax100-fac50-20.0		
% zscore -> nmf-user--itemax50-fac150-20.0
% first -> nmf-user--itemax100-fac50-20.0
% ceil => nmf-user--itemax100-fac100-20.0
% last => nmf-user--itemax100-fac100-20.0
% smoothed first => nmf-user--itemax100-fac50-20.0
% smoothed ceil => nmf-user--itemax100-fac50-20.0
% smoothed last => nmf-user--itemax100-fac100-20.0
 & \algname{\color{green}NMF} & 0.0005 & 0.0004 & \bf{0.0068} & \bf{0.0030} & \bf{0.0018} & & \bf{0.0009} & \bf{0.0006} & \bf{0.0007} \\
% zscore => nmf-item--itemax100-fac50-20.0
% first => nmf-item--itemax100-fac50-20.0
% ceil,last => nmf-item--itemax100-fac150-20.0
% smoothed first,ceil => nmf-item--itemax100-fac50-20.0
% smoothed last => nmf-item--itemax100-fac150-20.0
 &  &  & 0.0006 & \bf{0.0026} & \bf{0.0024} & \bf{0.0031} & & \bf{0.0010} & \bf{0.0009} & \bf{0.0010} \\


% rate => slim-item-itemsim-cos-knn50-itemax30-l17-l20.05-20.0
% zscore => slim-user-itemsim-cos-knn50-itemax100-l15-l20.5-20.0
% first,ceil => slim-user-itemsim-cos-knn100-itemax30-l10.5-l20.5-20.0
% last => slim-user-itemsim-cos-knn50-itemax50-l10.5-l20.5-20.0
 & \algname{SLIM} & 0.318 & 0.287 & 0.319 & 0.319 & 0.319 & &  &  &  \\
% zscore => like above
% first,ceil => like above
% last => like above
% smoothed first,last => slim-item-itemsim-cos-knn50-itemax100-l15-l25-20.0
% smoothed ceil => slim-item-itemsim-cos-knn100-itemax100-l15-l25-20.0
 &  &  & 0.305 & 0.319 & 0.319 & 0.319 & & 0.011 & 0.012 & 0.013 \\


\cline{1-11}


 \multirow{7}{*}{ML1M} & \algname{UserKNN} &  &  &  &  &  & &  &  &  \\
 &  &  &  &  &  &  & &  &  &  \\
  
 %\cline{1-14}
 
 & \algname{ItemKNN} &  &  &  &  &  & &  &  &  \\

%\cline{1-14}

 & \algname{BiasedMF} &  &  &  &  &  & &  &  &  \\
  
%\cline{1-14}
 & \algname{ListRank} &  &  &  &  &  & &  &  &  \\

%\cline{1-14}

 & \algname{SVD++} &  &  &  &  &  & &  &  &  \\

%\cline{1-14}

 & \algname{NMF} &  &  &  &  &  & &  &  &  \\
  
%\cline{1-14}
 & \algname{SLIM} &  &  &  &  &  & &  &  &  \\


\cline{1-11}


% all => userknn-user-usersim-pcc-shrink20-knn10-20.0
 \multirow{7}{*}{Yelp} & \algname{UserKNN} & 0.027 & 0.027 & 0.026 & 0.026 & 0.026 & &  &  &  \\
  
 %\cline{1-14}
% all => itemknn-item-itemsim-cos-shrink10-knn200-20.0
 & \algname{ItemKNN} & 0.043 & 0.043 & 0.042 & 0.043 & 0.043 & &  &  &  \\
 &  &  &  &  &  &  & &  &  &  \\

%\cline{1-14}

 & \algname{BiasedMF} &  &  &  &  &  & &  &  &  \\
  
%\cline{1-14}
% rate => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.005-fac150-20.0
% zscore => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.001-fac100-20.0
% first => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
% ceil,last => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
 & \algname{ListRank} & 0.020 & 0.019 & 0.018 & 0.019 & 0.019 & &  &  &  \\

%\cline{1-14}

 & \algname{SVD++} &  &  &  &  &  & &  &  &  \\

%\cline{1-14}

 & \algname{NMF} &  &  &  &  &  & &  &  &  \\
  
%\cline{1-14}
 & \algname{SLIM} &  &  &  &  &  & &  &  &  \\

 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/ndcg_table2_draft.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
%\captionof{table}{Performance of recommendation algorithms at nDCG@10 } \label{tab:res1}
\begin{tabular}{llrrrrrrrrrrr}
\toprule

 %\bottomrule

%\multirow{8}{*}{FilmTrust} & \algname{ItemAVG} & 0.0008 & 0.0004 & 0.0002 & 0.0001 & 0.0002 & 0.0005 & &  &  &  &  \\
  
 %\cline{1-14}
% all -> userknn-user-usersim-pcc-shrink20-knn200-20.0 
 \multirow{9}{*}{FilmTrust} & \algname{\color{red}UserKNN} & 0.543 & 0.544 & 0.543 & 0.542 & 0.542 & 0.542 & & 0.543 & 0.543 & 0.544 & 0.543 \\
  
 %\cline{1-14}
 % rate,zscore,first => itemknn-user-itemsim-cos-shrink20-knn30-20.0
 % floor,ceil => itemknn-user-itemsim-cos-shrink20-knn200-20.0
 % last => itemknn-user-itemsim-cos-shrink20-knn70-20.0
 % smoothed => itemknn-user-itemsim-cos-shrink20-knn40-20.0
 & \algname{\color{red}ItemKNN} & 0.537 & 0.557 & 0.514 & 0.496 & 0.502 & 0.483 & & 0.533 & 0.529 & 0.531 & 0.528 \\

% zscore => itemknn-item-itemsim-cos-shrink20-knn10-20.0
% first,ceil => itemknn-item-itemsim-cos-shrink20-knn50-20.0
% floor,last => itemknn-item-itemsim-cos-shrink20-knn40-20.0
% smoothed first,last => itemknn-item-itemsim-cos-shrink20-knn40-20.0
% smoothed floor,ceil => itemknn-item-itemsim-cos-shrink20-knn70-20.0
&  &  & 0.563 & 0.503 & 0.503 & 0.502 & 0.489 & & 0.496 & 0.498 & 0.497 & 0.485 \\


%\cline{1-14}
%rate => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% User-based transformation
% zscore => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% first => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0
% floor,ceil -> biasedmf-user-u0.001-i0.001-bias0.001-itemax30-itelearn0.0001-fac50-20.0
% last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% smoothed first -> biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0 
% smoothed floor,ceil,last => biasedmf-user-u0.0001-i0.0001-bias0.0001-itemax30-itelearn0.0001-fac100-20.0
 & \algname{BiasedMF} & 0.078 & 0.092 & \bf{0.317} & \bf{0.297} & \bf{0.314} & \bf{0.302} & & \bf{0.352} & \bf{0.342} & \bf{0.345} & \bf{0.335} \\
 
% first,ceil => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0 
% zscore => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.005-fac50-20.0
% floor => biasedmf-item-u0.001-i0.001-bias0.001-itemax100-itelearn0.0001-fac50-20.0
% last, smoothed last => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% smoothed first,ceil => biasedmf-item-u0.0001-i0.0001-bias0.0001-itemax100-itelearn0.0001-fac50-20.0
 &  &  & 0.167 & \bf{0.215} & \bf{0.243} & \bf{0.234} & \bf{0.270} & & \bf{0.174} &  & \bf{0.197} & \bf{0.230} \\
 
 
  
%\cline{1-14}
% rate => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac100-20.0
% zscore => listrankmf-user-u0.005-i0.005-itemax30-itelearn0.001-fac50-20.0
% first,ceil,last => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac150-20.0
% floor => listrankmf-user-u0.005-i0.005-itemax30-itelearn0.005-fac100-20.0
% smoothed first,last => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac150-20.0
% smoothed floor,ceil => listrankmf-user-u0.01-i0.01-itemax30-itelearn0.0001-fac100-20.0
 & \algname{\color{red}ListRank} & 0.412 & 0.459 & 0.393 & 0.375 & 0.382 & 0.380 & & 0.394 & 0.394 & 0.397 & 0.412 \\

% zscore => listrankmf-item-u0.001-i0.001-itemax30-itelearn0.01-fac50-20.0
% first => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac50-20.0
% floor => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac150-20.0
% ceil => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac150-20.0
% last => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.001-fac50-20.0
% smoothed first,last => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.0001-fac50-20.0
% smoothed floor,ceil => listrankmf-item-u0.005-i0.005-itemax30-itelearn0.001-fac50-20.0
 &  &  & 0.448 & 0.445 & 0.432 & 0.457 & 0.397 & & 0.455 & 0.423 & 0.395 & 0.422 \\

%\cline{1-14}
% rate => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% zscore => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac150-20.0
% first => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
% floor,ceil => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
% last => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax100-itelearn0.001-fac50-20.0
% smoothed => svdpp-user--u0.005-i0.005-impItem0.005-bias0.005-itemax30-itelearn0.001-fac50-20.0
 & \algname{SVD++} & 0.049 & 0.072 & \bf{0.079} & \bf{0.092} & \bf{0.087} & \bf{0.124} & & \bf{0.081} & \bf{0.092} & \bf{0.092} & \bf{0.102} \\

% zscore => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax100-itelearn0.001-fac50-20.0
% first => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.0001-fac100-20.0
% floor,ceil = > svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax50-itelearn0.0001-fac50-20.0                           
% last => svdpp-item--u0.0001-i0.0001-impItem0.0001-bias0.0001-itemax30-itelearn0.0001-fac50-20.0  
% smoothed all => svdpp-item--u0.001-i0.001-impItem0.001-bias0.001-itemax30-itelearn0.0001-fac50-20.0
 &  &  & 0.091 & \bf{0.193} & \bf{0.231} & \bf{0.222} & \bf{0.228} & & \bf{0.080} & \bf{0.126} & \bf{0.107} & \bf{0.143} \\

%\cline{1-14}
% rate -> nmf-user--itemax100-fac50-20.0		
% zscore -> nmf-user--itemax50-fac150-20.0
% first -> nmf-user--itemax100-fac50-20.0
% floor => nmf-user--itemax100-fac100-20.0
% ceil => nmf-user--itemax100-fac100-20.0
% last => nmf-user--itemax100-fac100-20.0
% smoothed first => nmf-user--itemax100-fac50-20.0
% smoothed floor => nmf-user--itemax100-fac100-20.0
% smoothed ceil => nmf-user--itemax100-fac50-20.0
% smoothed last => nmf-user--itemax100-fac100-20.0
 & \algname{\color{green}NMF} & 0.0005 & 0.0004 & \bf{0.0068} & \bf{0.0036} & \bf{0.0030} & \bf{0.0018} & & \bf{0.0009} & \bf{0.0007} & \bf{0.0006} & \bf{0.0007} \\
  
% zscore => nmf-item--itemax100-fac50-20.0
% first,floor => nmf-item--itemax100-fac50-20.0
% ceil,last => nmf-item--itemax100-fac150-20.0
% smoothed first,floor,ceil => nmf-item--itemax100-fac50-20.0
% smoothed last => nmf-item--itemax100-fac150-20.0
 &  &  & 0.0006 & \bf{0.0026} & \bf{0.0026} & \bf{0.0024} & \bf{0.0031} & & \bf{0.0010} & \bf{0.0009} & \bf{0.0009} & \bf{0.0010} \\


%\cline{1-14}
% rate => slim-item-itemsim-cos-knn50-itemax30-l17-l20.05-20.0
% zscore => slim-user-itemsim-cos-knn50-itemax100-l15-l20.5-20.0
% first,floor,ceil => slim-user-itemsim-cos-knn100-itemax30-l10.5-l20.5-20.0
% last => slim-user-itemsim-cos-knn50-itemax50-l10.5-l20.5-20.0
 & \algname{SLIM} & 0.318 & 0.287 & 0.319 & 0.319 & 0.319 & 0.319 & &  &  &  &  \\

% zscore => like above
% first,floor,ceil => like above
% last => like above
% smoothed first,last => slim-item-itemsim-cos-knn50-itemax100-l15-l25-20.0
% smoothed floor,ceil => slim-item-itemsim-cos-knn100-itemax100-l15-l25-20.0
 &  &  & 0.305 & 0.319 & 0.319 & 0.319 & 0.319 & & 0.011 & 0.012 & 0.012 & 0.013 \\
\cline{1-13}

%\multirow{8}{*}{ML1M} & \algname{ItemAVG} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
 
 \multirow{7}{*}{ML1M} & \algname{UserKNN} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
 
 & \algname{ItemKNN} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}

 & \algname{BiasedMF} &  &  &  &  &  &  & &  &  &  &  \\
  
%\cline{1-14}
 & \algname{ListRank} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}

 & \algname{SVD++} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}

 & \algname{NMF} &  &  &  &  &  &  & &  &  &  &  \\
  
%\cline{1-14}
 & \algname{SLIM} &  &  &  &  &  &  & &  &  &  &  \\

\cline{1-13}

%\multirow{8}{*}{Yelp} & \algname{ItemAVG} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
 
 \multirow{7}{*}{Yelp} & \algname{UserKNN} &  &  &  &  &  &  & &  &  &  &  \\
  
 %\cline{1-14}
 
 & \algname{ItemKNN} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}

 & \algname{BiasedMF} &  &  &  &  &  &  & &  &  &  &  \\
  
%\cline{1-14}
% rate => listrankmf-user-u0.001-i0.001-itemax50-itelearn0.005-fac150-20.0
% zscore => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.001-fac100-20.0
% first => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
% ceil,last => listrankmf-user-u0.001-i0.001-itemax30-itelearn0.005-fac150-20.0
 & \algname{ListRank} & 0.020 & 0.019 & 0.018 &  & 0.019 & 0.019 & &  &  &  &  \\

%\cline{1-14}

 & \algname{SVD++} &  &  &  &  &  &  & &  &  &  &  \\

%\cline{1-14}

 & \algname{NMF} &  &  &  &  &  &  & &  &  &  &  \\
  
%\cline{1-14}
 & \algname{SLIM} &  &  &  &  &  &  & &  &  &  &  \\

 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/table1.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{Yelp}} & & \multicolumn{5}{c}{\bf{ML1M}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{BiasedMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{SVD++} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{NMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/table10.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{Yelp}} & & \multicolumn{5}{c}{\bf{ML1M}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{BiasedMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{SVD++} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{NMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/table11.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{CiaoDVD}} & & \multicolumn{5}{c}{\bf{FilmTrust}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{BiasedMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{SVD++} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{NMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}





==> results-presentation/table12.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{BX}} & & \multicolumn{5}{c}{\bf{Epinions}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{BiasedMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{SVD++} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{NMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  
%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}

==> results-presentation/table2.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{CiaoDVD}} & & \multicolumn{5}{c}{\bf{FilmTrust}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{BiasedMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{SVD++} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{NMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}





==> results-presentation/table3.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{BX}} & & \multicolumn{5}{c}{\bf{Epinions}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{BiasedMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{SVD++} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{NMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_u$ & & &  &  &  & & & &  &  &  & \\

%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}

==> results-presentation/table4.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{Yelp}} & & \multicolumn{5}{c}{\bf{ML1M}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{BiasedMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{SVD++} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{NMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/table5.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{CiaoDVD}} & & \multicolumn{5}{c}{\bf{FilmTrust}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{BiasedMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{SVD++} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{NMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}





==> results-presentation/table6.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{BX}} & & \multicolumn{5}{c}{\bf{Epinions}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{BiasedMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{SVD++} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

\cline{1-14}

 \algname{NMF} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_i$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_i$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_i$ & & &  &  &  & & & &  &  &  & \\
  & $last_i$ & & &  &  &  & & & &  &  &  & \\
  & rating & & &  &  &  & & & &  &  &  & \\
  & $zscore_i$ & & &  &  &  & & & &  &  &  & \\

%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}

==> results-presentation/table7.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\small
\centering
\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{Yelp}} & & \multicolumn{5}{c}{\bf{ML1M}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{BiasedMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{SVD++} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{NMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}


==> results-presentation/table8.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{CiaoDVD}} & & \multicolumn{5}{c}{\bf{FilmTrust}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{BiasedMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{SVD++} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{NMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}





==> results-presentation/table9.tex <==
%\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\vspace*{-5pt}
\small
\centering
%\captionof{table}{Long-tail and catalog coverage of recommendation algorithms at top-N=10 and cutting point of 20\% for determining long-tail items } \label{tab:res1}
\begin{tabular}{llrrlllrrrlllr}
\toprule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{inputs} & \multicolumn{5}{c}{\bf{BX}} & & \multicolumn{5}{c}{\bf{Epinions}} \\\cline{3-7}\cline{9-13}
  
 
 & & \multicolumn{2}{c}{params} & CC & LTC & nDCG & & \multicolumn{2}{c}{params} & CC & LTC & nDCG \\
 \bottomrule
 
 \algname{ItemAVG} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{UserKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
 \cline{1-14}
 
  \algname{ItemKNN} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{BiasedMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
 \algname{ListRank} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{SVD++} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}

 \algname{NMF} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
\cline{1-14}
\algname{SLIM} & $first_u$ & \multirow{1}{*}{20} & \multirow{1}{*}{-} &  &  &  & & \multirow{1}{*}{50} & \multirow{1}{*}{-} &  &  &  & \\
  & $floor_u$ & & &  &  &  & & & &  &  &  & \\
  & $ceil_u$ & & &  &  &  & & & &  &  &  & \\
  & $last_u$ & & &  &  &  & & & &  &  &  & \\
  
%\cline{1-19}

  %\algname{WRMF} & $Per_i$ & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} & & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \bf{} & \bf{} & \bf{} \\
  %& rating & & &  &  &  & & & & &  &  & & & & & &  \\
 
 \bottomrule
\end{tabular}
\end{table*}
